State of What Art? A Call for Multi-Prompt LLM Evaluation

Recent advances in large language models (LLMs) have led to the development of various evaluation benchmarks. These benchmarks typically rely on a single instruction template for evaluating all LLMs on a specific task. In this paper, we comprehensively analyze the brittleness of results obtained via single-prompt evaluations across 6.5M instances, involving 20 different LLMs and 39 tasks from 3 benchmarks. To improve robustness of the analysis, we propose to evaluate LLMs with a set of diverse prompts instead. We discuss tailored evaluation metrics for specific use cases (e.g., LLM developers vs. developers interested in a specific downstream task), ensuring a more reliable and meaningful assessment of LLM capabilities. We then implement these criteria and conduct evaluations of multiple models, providing insights into the true strengths and limitations of current LLMs.

==> sections/09_limitations.tex <==
TODO

==> tables/average_rank_per_metric.tex <==
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\hline
\textbf{}                & \textbf{average} & \textbf{maximum} & \textbf{saturation} & \textbf{combined} \\ \hline
\textbf{\tzero{}}          & 7.45             & 7.59             & 6.00                & 7.41              \\
\textbf{\tzeropp{}}            & 5.18             & 6.28             & \textbf{4.08}          & 5.10              \\
\textbf{\falcon{}}       & 6.88             & 7.12             & 5.36                & 6.80              \\
\textbf{\mpt{}}          & 8.76             & 8.96             & 7.80                & 8.80              \\
\textbf{\alpacasmall{}}       & 7.92             & 5.83             & 7.63                & 7.88              \\
\textbf{\alpacabig{}}      & 5.51             & 4.92             & 5.13                & 5.72              \\
\textbf{\flansmall{}}   & 6.71             & 7.38             & 5.00                & 6.63              \\
\textbf{\flanbase{}}    & 6.17             & 6.67             & 4.86                & 6.08              \\
\textbf{\flanlarge{}}   & 4.25             & 5.17             & 4.79                & 4.29              \\
\textbf{\flanxl{}}      & 2.69             & 3.10             & 4.51                & 2.85              \\
\textbf{\flanxxl{}}     & \textbf{1.46}     & \textbf{1.87}       & 4.44                & \textbf{1.56}        \\
\textbf{\airoboros{}}   & 5.73             & 5.87             & 6.13                & 5.67              \\
\textbf{\noushermes{}} & 7.00             & 5.47             & 8.13                & 6.87              \\
\textbf{\ultralm{}}     & 8.60             & 6.60             & \underline{8.93}       & 8.40              \\
\textbf{\vicuna{}}      & 3.13             & 3.13             & 5.33                & 3.33              \\
\textbf{\minotaur{}}    & \underline{10.67}   & \underline{9.67}    & 8.67                & \underline{10.27}    \\ \hline
\end{tabular}%
}
\caption{\label{tab:model_rankings_avg} 
\mnote{old average rank per metric table} Bold numbers indicate the best averaged rank per metric, while underlined numbers indicate the worst averaged rank per metric.
}
\end{table}

==> tables/average_rank_per_metric_new.tex <==
\remove{
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\hline
\textbf{}                & \textbf{average}    & \textbf{maximum}    & \textbf{saturation} & \textbf{combined}   \\ \hline
\textbf{t0\_3b}          & 7.40                & \underline{12.2}       & 5.9                 & 7.9                 \\
\textbf{t0++}            & 6.32                & 8.00                & 5.08                & 6.20                \\
\textbf{falcon-7b}       & 7.48                & 7.76                & 6.68                & 7.32                \\
\textbf{mpt-7b}          & 9.52                & 10.04               & 8.80                & 9.72                \\
\textbf{alpaca-7b}       & \underline{13.9}       & 7.90                & \underline{13.6}       & \underline{13.2}       \\
\textbf{alpaca-13b}      & 7.32                & 5.80                & 7.32                & 7.40                \\
\textbf{flan-t5-small}   & 6.20                & 9.60                & 7.90                & 5.90                \\
\textbf{flan-t5-base}    & 8.00                & 10.50               & 6.50                & 8.20                \\
\textbf{flan-t5-large}   & 4.10                & 8.50                & 4.80                & 4.50                \\
\textbf{flan-t5-xl}      & 2.72                & 3.16                & 4.68                & 3.08                \\
\textbf{flan-t5-xxl}     & {\underline{ \textbf{1.40}}} & {\underline{\textbf{2.36}}} & {\underline{\textbf{3.40}}} & {\underline{\textbf{1.48}}} \\
\textbf{airoboros-13b}   & 7.24                & 7.48                & 7.28                & 7.60                \\
\textbf{nous-hermes-13b} & 7.68                & 5.76                & 8.76                & 7.56                \\
\textbf{ultralm-13b}     & 10.04               & 7.88                & 8.96                & 9.48                \\
\textbf{vicuna-13b}      & 6.56                & 3.36                & 9.04                & 6.52                \\
\textbf{minotaur-15b}    & 11.88               & 9.88                & 8.52                & 11.76               \\ \hline
\end{tabular}%
}
\caption{\label{tab:model_rankings_avg_new} 
\mnote{new average rank per metric table}
Bold numbers indicate the best averaged rank per metric, while underlined numbers indicate the worst averaged rank per metric.
}
\end{table}
}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\hline
\textbf{}                & \textbf{average}    & \textbf{maximum}    & \textbf{saturation} & \textbf{combined}   \\ \hline
\textbf{t0\_3b}          & 7.40                & \underline{12.20}       & 5.90                 & 7.90                 \\
\textbf{t0++}            & 4.80                & 8.80                & 4.20                & 4.63                \\
\textbf{falcon-7b}       & 9.40                & 8.00                & 9.70                & 8.27                \\
\textbf{mpt-7b}          & 10.30               & 11.10               & 10.00               & 10.00               \\
\textbf{alpaca-7b}       & \underline{13.90}       & 7.90                & 13.60       & 13.20      \\
\textbf{alpaca-13b}      & 11.50                & 6.60                & 12.40               & 10.72               \\
\textbf{flan-t5-small}   & 6.20                & 9.60                & 7.90                & 5.90                \\
\textbf{flan-t5-base}    & 8.00                & 10.50               & 6.50                & 8.20                \\
\textbf{flan-t5-large}   & 4.10                & 8.50                & 4.80                & 4.50                \\
\textbf{flan-t5-xl}      & 2.80                & 4.20                & 5.80                & 3.72                \\
\textbf{flan-t5-xxl}     & {{\textbf{1.40}}} & {{\textbf{3.10}}} & {{\textbf{3.70}}} & {{\textbf{1.72}}} \\
\textbf{airoboros-13b}   & 9.50                & 10.20               & 9.50                & 10.36               \\
\textbf{nous-hermes-13b} & 8.90                & 6.30                & 9.70                & 8.73                \\
\textbf{ultralm-13b}     & 12.30               & 9.80                & 9.30                & 11.09               \\
\textbf{vicuna-13b}      & 11.80               & 3.70                & \underline{14.70}               & 10.63               \\
\textbf{minotaur-15b}    & 13.70               & 10.20               & 8.30                & \underline{13.63}               \\ \hline
\end{tabular}%
}\caption{\label{tab:model_rankings_avg_new_lmentry} Average model ranks for each metric across all tasks in \lmentry{}. 
Bold numbers indicate the best averaged rank per metric, while underlined numbers indicate the worst averaged rank per metric.
}
\end{table}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\hline
\textbf{}                & \textbf{average}    & \textbf{maximum}    & \textbf{saturation} & \textbf{combined}   \\ \hline
\textbf{t0++}            & 7.33                & 7.47                & 5.67                & 7.33                \\
\textbf{falcon-7b}       & 6.20                & 7.60                & 4.67                & 6.47                \\
\textbf{mpt-7b}          & 9.00                & 9.33                & 8.00                & 9.53                \\
\textbf{alpaca-13b}      & 4.53                & 5.27                & 3.93                & 4.67                \\
\textbf{flan-t5-xl}      & 2.67                & 2.47                & 3.93                & 2.67                \\
\textbf{flan-t5-xxl}     & {{\textbf{1.40}}} & {{\textbf{1.87}}} & {{\textbf{3.20}}} & {{\textbf{1.33}}} \\
\textbf{airoboros-13b}   & 5.73                & 5.67                & 5.80                & 5.67                \\
\textbf{nous-hermes-13b} & 6.87                & 5.40                & 8.13                & 6.67                \\
\textbf{ultralm-13b}     & 8.53                & 6.60                & \underline{8.73}                & 8.20                \\
\textbf{vicuna-13b}      & 3.07                & 3.13                & 5.27                & 3.13                \\
\textbf{minotaur-15b}    & \underline{10.67}               & \underline{9.67}                & 8.67                & \underline{10.33 }              \\ \hline
\end{tabular}%
}\caption{\label{tab:model_rankings_avg_new_bbh} 
Average model ranks for each metric across all tasks in \bbh{}.
Bold numbers indicate the best averaged rank per metric, while underlined numbers indicate the worst averaged rank per metric.
}
\end{table}

==> tables/bmk_scores.tex <==
\begin{table}[t!]
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{l}{}        & \multicolumn{2}{c}{\textbf{MMLU}}     & \multicolumn{2}{c}{\textbf{BBL}}      & \multicolumn{2}{c}{\textbf{BBH}}      & \multicolumn{2}{c}{\textbf{SuperNatInst}} \\ \hline
\multicolumn{1}{l}{}        & \textbf{achievability} & \textbf{max} & \textbf{achievability} & \textbf{max} & \textbf{achievability} & \textbf{max} & \textbf{achievability}   & \textbf{max}   \\
\textbf{T5\_XXL}            & 0.54                   & 0.89         & 0.54                   & 0.89         & 0.54                   & 0.89         & 0.54                     & 0.89           \\
\textbf{T0++}               & 0.65                   & 0.87         & 0.65                   & 0.87         & 0.65                   & 0.87         & 0.65                     & 0.87           \\
\textbf{GPT3.5-fast}        & 0.83                   & 0.90         & 0.83                   & 0.90         & 0.83                   & 0.90         & 0.83                     & 0.90           \\
\textbf{Text-da-vinchi 002} & 0.77                   & 0.90         & 0.77                   & 0.90         & 0.77                   & 0.90         & 0.77                     & 0.90           \\
\textbf{Text-da-vinchi 003} & 0.81                   & 0.91         & 0.81                   & 0.91         & 0.81                   & 0.91         & 0.81                     & 0.91           \\
\textbf{MPT7b}              & 0.79                   & 0.82         & 0.79                   & 0.82         & 0.79                   & 0.82         & 0.79                     & 0.82           \\
\textbf{RedPajama7b}        & 0.78                   & 0.89         & 0.78                   & 0.89         & 0.78                   & 0.89         & 0.78                     & 0.89           \\
\textbf{FLAN\_Alpaca\_GPT4} & 0.82                   & 0.90         & 0.82                   & 0.90         & 0.82                   & 0.90         & 0.82                     & 0.90           \\ \hline
\end{tabular}
\caption{Average difference from monolingual baselines (higher is better) calculated on MRR scores. Our teacher-student model achieves better results overall in both shared and diverse scripts. It is otherwise between the baselines, except for shared script, where it is better for \lowres{}.}
\label{tab:bmk_scores}
\end{table}

==> tables/bmk_stability.tex <==
\begin{table}[t!]
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{}               & \multicolumn{1}{l}{\textbf{MMLU}} & \multicolumn{1}{l}{\textbf{BBH}} & \multicolumn{1}{l}{\textbf{BBL}} & \multicolumn{1}{l}{\textbf{LMentry}} & \multicolumn{1}{l}{\textbf{SuperNatInst}} \\ \midrule
\textbf{\#permutations} & 12                                & 27                               & 13                               & 15                                   & 26                                        \\
\textbf{rank\%}         & 60                                & 23                               & 63                               & 61                                   & 42                                        \\ \bottomrule
\end{tabular}
\caption{Average difference from monolingual baselines (higher is better) calculated on MRR scores. Our teacher-student model achieves better results overall in both shared and diverse scripts. It is otherwise between the baselines, except for shared script, where it is better for \lowres{}.}
\label{tab:bmk_stability}
\end{table}

==> tables/kendall_and_anova_table.tex <==
\begin{table*}[tb!]
\centering
% \small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcclccccc}
% \hline \textbf{Benchmark} & 
\toprule
\textbf{Benchmark \& Task} & \textbf{\# default}  & \textbf{\# paraphrases} & \textbf{Source} & \textbf{Method} & \textbf{Samples} & \textbf{Kendall's W} & \textbf{Friedman p-val}& \textbf{\# Models}
\\ \hline
\textbf{\lmentry{}}  \\
 $\quad$ all words from category & 3  & 255 & auto & 0-shot & 100 & \textbf{.622} &  & 11\\
 $\quad$ any words from category & 3 & 256 & auto & 0-shot & 100 & .471 &  &11\\
 $\quad$ ends with word & 3 & 223 & auto & 0-shot & 100 & .418 &  & 11\\
 $\quad$ first alphabetically & 3 & 231 & auto & 0-shot & 100 & .397 &  & 11\\
 $\quad$ homophones & 3 & 262 & auto & 0-shot & 100 & .588 &  & 11\\
 $\quad$ less letters & 3 & 237 & auto & 0-shot & 100 & .479 &  & 11\\
 $\quad$ more letters & 3 & 234 & auto & 0-shot & 100 & .526 &  & 11\\
 $\quad$ rhyming word & 3 & 242 & auto & 0-shot & 100 & .504 &  & 11\\
 $\quad$ word before & 3 & 230 & auto & 0-shot & 100 & .515 &  & 11\\
 $\quad$ word not containing & 3 & 231 & auto & 0-shot & 100 & \underline{.333} &  & 11\\
  
\midrule

\textbf{\bigbenchlite{}} \\ 
$\quad$ bbq lite & 1 & 12 & human & 0-shot & all & .890 &  & 9\\
$\quad$ code line description & 1 & 9 & human & 0-shot & all & .756 &  & 9\\
$\quad$ conceptual combinations & 1 & 8 & human & 0-shot & all & .731 &  & 9\\
$\quad$ hindu knowledge & 1 & 7 & human & 0-shot & all & .560 &  & 9\\
$\quad$ known unknown & 1 & 7 & human & 0-shot & all & \underline{.316} &  & 9\\
$\quad$ language identification & 1 & 8 & human & 0-shot & all & .811 &  & 9\\
$\quad$ logic grid puzzle & 1 & 8 & human & 0-shot & all & .796 &  & 9\\
$\quad$ logical deduction & 1 & 9 & human & 0-shot & all & \textbf{.913} &  & 9\\
$\quad$ novel concepts & 1 & 10 & human & 0-shot & all & .787 &  & 9\\
$\quad$ play dialog & 1 & 10 & human & 0-shot & all & .355 &  & 9\\
$\quad$ strange stories & 1 & 10 & human & 0-shot & all & .731 &  & 9\\
$\quad$ strategic qa & 1 & 9 & human & 0-shot & all & .529 &  & 9\\
$\quad$ vitaminc fact verification & 1 & 10 & human & 0-shot & all & .888 &  & 9\\
$\quad$ winowhy & 1 & 10 & human & 0-shot & all & .520 &  & \\

\midrule

\textbf{\bigbenchhard{}} \\ 
$\quad$ causal judgement  & 1  & 186 & auto & 1-shot & 100 & \textbf{.857} &  & 11\\
$\quad$ disambiguation qa  & 1  & 187 & auto & 1-shot & 100 & .756 &  & 11\\
$\quad$ formal fallacies  & 1  & 183 & auto & 1-shot & 100 & \underline{.566} &  & 11\\
$\quad$ geometric shapes  & 1  & 177 & auto & 1-shot & 100 & .698 &  & 11\\
$\quad$ hyperbaton  & 1  & 154 & auto & 1-shot & 100 & .700 &  & 11\\
$\quad$ logical deduction five objects  & 1  & 188 & auto & 1-shot & 100 & .804 &  & 11\\
$\quad$ logical deduction seven objects  & 1  & 185 & auto & 1-shot & 100 & .760 &  & 11\\
$\quad$ logical deduction three objects  & 1  & 186 & auto & 1-shot & 100 & .744 &  & 11\\
$\quad$ movie recommendation  & 1  & 179 & auto & 1-shot & 100 & .623 & & 11\\
$\quad$ navigate  & 1  & 169 & auto & 1-shot & 100 & .779 &  & 11\\
$\quad$ penguins in a table  & 1  & 182 & auto & 1-shot & 100 & .830 &  & 11\\
$\quad$ ruin names  & 1  & 156 & auto & 1-shot & 100 & .741 &  & 11\\
$\quad$ salient translation error detection  & 1  & 135 & auto & 1-shot & 100 & .771 &  & 11\\
$\quad$ snarks  & 1  & 161 & auto & 1-shot & 100 & .811 &  & 11\\
$\quad$ sports understanding  & 1  & 172 & auto & 1-shot & 100 & .628 &  & 11\\

\bottomrule
\end{tabular}
}
\caption{\label{tab:tasks_info} 
Bold numbers indicate the maximal value for Kendall's $W \in [0,1]$ per benchmark, while underlined numbers indicate the minimal Kendall's $W$ within that benchmark. The smaller the value of $W$ the more that the ranking on different prompts is de-correlated. Most $W$ are smaller than $0.85$, indicating less than optimal correlation. The p-values from Friedman test indicate that the difference between rankings of models when using different prompts is significant.  
 \gabis{remove leading zero, put only two percision point, always have two digits, even if trailing zero. For the BBL tasks, let's write the actual number of samples, instead of ``All''. Should we order each benchmark from most agreement to least agreement according to Kendall's $W$? I'd remove the ``default'' column}\rotem{good idea about the sorting based on W values, let's do it after we update the F and p-values from the ANOVA}
}
\end{table*}

==> tables/kendall_bbl.tex <==
\begin{table}[!htbp]
% \centering
% \small
\resizebox{1.01\columnwidth}{!}{%
\begin{tabular}{lccc}
% \hline \textbf{Benchmark} & 
\toprule
\textbf{Benchmark \& Task} & \textbf{Kendall's W} & \textbf{Friedman p-val}
\\ \hline

\textbf{\bigbenchlite{}} \\ 
$\quad$ known unknown &  .316 & \textbf{4.4E-5}\\
$\quad$ play dialog &  .355 & \textbf{4.3E-5}\\
$\quad$ winowhy &   .520 & \textbf{6.0E-4}\\
$\quad$ strategic qa &  .529 & .191\\
$\quad$ hindu knowledge &   .560 & .569\\
$\quad$ conceptual combinations &   .731 & .132\\
$\quad$ strange stories & .731 & .431\\
$\quad$ code line description &   .756 & \textbf{.002}\\
$\quad$ novel concepts &  .787 & .620\\
$\quad$ logic grid puzzle &  .796 & \textbf{.010}\\
$\quad$ language identification &   .811 & \textbf{.002}\\
$\quad$ vitaminc fact verification &  .888 & .772\\
$\quad$ bbq lite &  .890 & \textbf{.023}\\
$\quad$ logical deduction &  .913 & .895\\

\bottomrule
\end{tabular}
}
\caption{\label{tab:tasks_info2lite} 
Kendall's $W \in [0,1]$ values for all tasks sorted in ascending order. The smaller the value of $W$ the more that the ranking on different prompts is de-correlated. Most $W$ are smaller than $0.85$, indicating less than optimal correlation. The p-values from the Friedman test indicate significant differences between rankings of models when using different prompts for 7 tasks. 
}
\end{table}


==> tables/metric_ranking_comparisson.tex <==
\begin{table}[!htbp]
% \centering
% \small
\resizebox{1.02\columnwidth}{!}{%
\begin{tabular}{lcccc}
% \hline \textbf{Benchmark} & 
\toprule
\textbf{Benchmark \& Task} & \textbf{MaxP} & \textbf{AvgP}& \textbf{Sat} & \textbf{Combined}
\\ \hline
\textbf{\lmentry{}}  \\
 $\quad$ all words from category & .958 & .967 & .950 & .900\\
 $\quad$ any words from category & .979 & .967 & .983 & .983\\
 $\quad$ ends with word &  .104 & .967 & .050 & .517\\
 $\quad$ first alphabetically  & 1.00 & .950 & .933 & .950\\
 $\quad$ homophones  & .945 & 1.00 & .900 & .933\\
 $\quad$ less letters  & .983 & 1.00 & .917 & .967\\
 $\quad$ more letters  & .970 & .983 & .917 & .983\\
 $\quad$ rhyming word  & 1.00 & .967 & .983 & .967\\
 $\quad$ word before  & 1.00 & 1.00 & .983 & 1.00\\
 $\quad$ word not containing  & .836 & .967 & .783 & .850\\
  
\midrule

\textbf{\bigbenchhard{}} \\ 
$\quad$ causal judgement  & 1.00 & 1.00 & 1.00 & 1.00\\
$\quad$ disambiguation qa  &  1.00 & 1.00 & .964 & 1.00\\
$\quad$ formal fallacies  &   .991 & .927 & .818 & .855\\
$\quad$ geometric shapes  & 1.00 & .964 & 1.00 & .964\\
$\quad$ hyperbaton  &  .953 & 1.00 & .927 & .964\\
$\quad$ logical deduction five objects  & 1.00 & .964 & .855 & .964\\
$\quad$ logical deduction seven objects  & 1.00 & 1.00 & .964 & .964\\
$\quad$ logical deduction three objects  &  1.00 & .964 & .891 & .964\\
$\quad$ movie recommendation  & .954 & .927 & .891 & .964\\
$\quad$ navigate  &   .964 & 1.00 & 1.00 & .964\\
$\quad$ penguins in a table  & 1.00 & 1.00 & .891 & 1.00\\
$\quad$ ruin names  & 1.00 & 1.00 & .964 & .891\\
$\quad$ salient translation error detection  & 1.00 & 1.00 & 1.00 & 1.00\\
$\quad$ snarks  & 1.00 & 1.00 & .964 & 1.00\\
$\quad$ sports understanding  & 1.00 & 1.00 & .964 & 1.00\\

\bottomrule
\end{tabular}
}
\caption{\label{tab:metric_rankings_comparisson} Kendall's Tau model ranking comparisons before and after removal of incorrect paraphrases. Results show near-perfect to perfect agreement across all tasks, except for \lmentry{}'s “ends with word” task.
}
% \mnote{DAN: we can cite this work https://aclanthology.org/2022.naacl-main.167.pdf as they say  "We find that models can learn just as fast with many prompts that are intentionally irrelevant or even pathologically misleading as they do with constructively “good” prompts.". this might also be inline with \citet{sun2023evaluating} (wrong templates similar to templates observed in training preformed as better instruction templates than correct and unobserved templates)}
\end{table}



==> tables/min_edit_dist_max_diff.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!t]{
\begin{adjustwidth}{-1cm}{-1cm}
% \resizebox{\textwidth}{!}{%
\centering
\small
\begin{tabular}{|p{1.1cm}|c|p{5cm}|c|p{5cm}|c|c|}
\toprule
\textbf{Change}               & \textbf{Model}     & \textbf{P1}                                                                                                       & \textbf{Acc.} & \textbf{P2}                                                                                                          & \textbf{Acc.} & \textbf{Diff.}               \\ \hline
`.' --\textgreater `:'        & nous-hermes    & Create a word that does not include the letter   ``\{letter\}''.                                                    & .04          & Create a word that does not include the letter   ``\{letter\}''\textbf{\textit{:}}                                                       & .65          & {\color[HTML]{00B050} +.62} \\
                              & alpaca-13b         & Create a sentence that concludes with the term   ``\{word\}''.                                                      & .61          & Create a sentence that concludes with the term   ``\{word\}''\textbf{\textit{:}}                                                         & .19          & {\color[HTML]{C00000} -.42} \\ \hline
+ `.'                       & alpaca-13b         & Write a word that lacks the letter ``\{letter\}''                                                                   & .04          & Write a word that lacks the letter ``\{letter\}''\textbf{\textit{.}}                                                                     & .42          & {\color[HTML]{00B050} +.38} \\
                              % & falcon-7b & Write a word that lacks the letter ``\{letter\}''                                                                   & .19          & Write a word that lacks the letter ``\{letter\}''\textbf{\textit{.}}                                                                     & .50          & {\color[HTML]{00B050} +.31} \\
                              & flan-t5-xl         & Write a word that omits the letter ``\{letter\}''                                                                   & .77          & Write a word that omits the letter ``\{letter\}''\textbf{\textit{.}}                                                                     & .54          & {\color[HTML]{C00000} -.23} \\ \hline
% + ``...''         & mpt-7b    & Write a word that does not contain the letter \textbf{\textit{\{letter\}}}.\textbackslash{}nWord:                                   & .58          & Write a word that does not contain the letter \textbf{\textit{``\{letter\}''}}.\textbackslash{}nWord:                                    & .19          & {\color[HTML]{C00000} -.38} \\
                              % & flan-t5-small      & Write a word that does not contain the letter \textit{\textbf{\textit{\{letter\}}}}.\textbackslash{}nWord:                                   & .62          & Write a word that does not contain the letter \textbf{\textit{``\{letter\}''}}.\textbackslash{}nWord:                                    & .04          & {\color[HTML]{C00000} -.58} \\
                              % & flan-t5-xl         & Write a word that excludes the letter \textbf{\textit{\{letter\}}}.                                                                 & .81          & Write a word that excludes the letter \textbf{\textit{``\{letter\}''}}.                                                                  & .23          & {\color[HTML]{C00000} -.58} \\ \hline
% + `Q:'         & minotaur       & Are all of the words in the set \{words\} classified as   \{category\}? Please respond with either 'yes' or 'no'. & .69          & \textbf{\textit{Q:}} Are all of the words in the set \{words\} classified as   \{category\}? Please respond with either 'yes' or 'no'. & .02          & {\color[HTML]{C00000} -.67} \\
                              % & airoboros     & Are all the words in \{words\} categorized as \{category\}? Please   answer with either 'yes' or 'no'.            & .75          & \textbf{\textit{Q:}} Are all the words in \{words\} categorized as \{category\}?   Please answer with either 'yes' or 'no'.            & .09          & {\color[HTML]{C00000} -.66} \\
                              % & mpt-7b    & Are all the words in \{words\} categorized as \{category\}? Please   answer with either 'yes' or 'no'.            & .57          & \textbf{\textit{Q:}} Are all the words in \{words\} categorized as \{category\}?   Please answer with either 'yes' or 'no'.            & .00          & {\color[HTML]{C00000} -.57} \\
                              % & t0pp               & Are all the words in \{words\} categorized as \{category\}? Please   answer with either 'yes' or 'no'.            & .99          & \textbf{\textit{Q:}} Are all the words in \{words\} categorized as \{category\}?   Please answer with either 'yes' or 'no'.            & .55          & {\color[HTML]{C00000} -.44} \\ \hline
+ `using'                   & flan-t5-large      & Your task is to write a word without the letter   ``\{letter\}''.                                                   & .46          & Your task is to write a word without \textbf{\textit{using}} the letter   ``\{letter\}''.                                                & .12          & {\color[HTML]{C00000} -.35} \\
                              & falcon-7b & Write a word without the letter \{letter\}.\textbackslash{}nOutput word:                                          & .12          & Write a word without \textbf{\textit{using}} the letter \{letter\}.\textbackslash{}nOutput word:                                       & .35          & {\color[HTML]{00B050} +.23} \\
                              % & flan-t5-large      & Write a word without the letter \{letter\}.\textbackslash{}nOutput word:                                          & .73          & Write a word without \textbf{\textit{using}} the letter \{letter\}.\textbackslash{}nOutput word:                                       & .50          & {\color[HTML]{C00000} -.23} \\ 
                              \hline
omits --\textgreater lacks    & ultralm-13b        & Write a word that \textbf{\textit{omits}} the letter ``\{letter\}''.                                                                  & .62          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''.                                                                     & .19          & {\color[HTML]{C00000} -.42} \\
                              % & falcon-7b & Write a word that \textbf{\textit{omits}} the letter ``\{letter\}''.                                                                  & .19          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''.                                                                     & .50          & {\color[HTML]{00B050} +.31} \\
                              & flan-t5-xl         & Write a word that \textbf{\textit{omits}} the letter ``\{letter\}''.                                                                  & .54          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''.                                                                     & .81          & {\color[HTML]{00B050} +.27} \\ \hline
\begin{tabular}[c]{@{}l@{}}contain \\ --\textgreater have\end{tabular}   & falcon-7b & Write a word that does not \textbf{\textit{contain}} the letter   ``\{letter\}''.                                                     & .81          & Write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                           & .19          & {\color[HTML]{C00000} -.62} \\
                              % & falcon-7b & Write a word that does not \textbf{\textit{contain}} the letter   ``\{letter\}''.                                                     & .81          & Write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                           & .27          & {\color[HTML]{C00000} -.54} \\
                              & flan-t5-xxl        & Please write a word that does not \textbf{\textit{contain}} the letter   ``\{letter\}''.                                              & .62          & Please write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                    & .88          & {\color[HTML]{00B050} +.27} \\ \hline
\begin{tabular}[c]{@{}l@{}}include \\ --\textgreater have\end{tabular}  & falcon-7b & Write a word that does not \textbf{\textit{include}} the letter   ``\{letter\}''.                                                     & .81          & Write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                           & .19          & {\color[HTML]{C00000} -.62} \\
                              & flan-t5-xl         & Write a word that does not \textbf{\textit{include}} the letter   ``\{letter\}''.                                                     & .42          & Write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                           & .73          & {\color[HTML]{00B050} +.31} \\
                              % & falcon-7b & Please write a word that does not \textbf{\textit{include}} the letter   ``\{letter\}''.                                              & .77          & Please write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                    & .35          & {\color[HTML]{C00000} -.42} \\
                              & ultralm-13b        & Please write a word that does not \textbf{\textit{include}} the letter   ``\{letter\}''.                                              & .46          & Please write a word that does not \textbf{\textit{have}} the letter   ``\{letter\}''.                                                    & .12          & {\color[HTML]{C00000} -.35} \\ \hline
excludes --\textgreater lacks & flan-t5-large      & Write a word that \textbf{\textit{excludes}} the letter ``\{letter\}''.                                                               & .54          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''.                                                                     & .12          & {\color[HTML]{C00000} -.42} \\
                              & flan-t5-xl         & Write a word that \textbf{\textit{excludes}} the letter ``\{letter\}''.                                                               & .19          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''.                                                                     & .81          & {\color[HTML]{00B050} +.62} \\
                              % & flan-t5-xl         & Write a word that \textbf{\textit{excludes}} the letter ``\{letter\}''                                                                & .46          & Write a word that \textbf{\textit{lacks}} the letter ``\{letter\}''                                                                      & .88          & {\color[HTML]{00B050} +.42} \\ 
                              \bottomrule
\end{tabular}% \\
\caption{Representative examples of instruction template pairs from \lmentry{} with very minor differences but notable variations in performance (open-source models).}
\label{tab:min_edit_dist_max_diff}
\end{adjustwidth}
}\end{table*}

==> tables/min_edit_distance_pairs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
                                 & \textbf{t03b}                 & \textbf{t0pp}                 & \textbf{fal7b}                & \textbf{mpt7b}                & \textbf{alp7b}                & \textbf{alp13b}               & \textbf{ft5-s}                & \textbf{ft5-b}                & \textbf{ft5-l}                & \textbf{ft5-xl}               & \textbf{ft5-xxl}              & \textbf{air13b}               & \textbf{nou13b}               & \textbf{ult13b}               & \textbf{vic13b}               & \textbf{min15b}               \\
{[}{]}-\textgreater{}.           & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{FBB6B7}-0.07 & \cellcolor[HTML]{7CC990}0.13  & \cellcolor[HTML]{EEF8F0}0.02  & \cellcolor[HTML]{FEFAFA}0.00  & \cellcolor[HTML]{63BE7B}0.16  & \cellcolor[HTML]{FDE4E4}-0.03 & \cellcolor[HTML]{FEFCFC}0.00  & \cellcolor[HTML]{FDE7E8}-0.02 & \cellcolor[HTML]{F98081}-0.13 & \cellcolor[HTML]{F7FCF9}0.01  & \cellcolor[HTML]{FEF9F9}-0.01 & \cellcolor[HTML]{FEEDED}-0.02 & \cellcolor[HTML]{C5E7CE}0.06  & \cellcolor[HTML]{FAFDFB}0.01  & \cellcolor[HTML]{F1F9F3}0.01  \\
. -\textgreater :                & \cellcolor[HTML]{FEFDFD}0.00  & \cellcolor[HTML]{CEEBD6}0.05  & \cellcolor[HTML]{F8FDF9}0.01  & \cellcolor[HTML]{F5FBF6}0.01  & \cellcolor[HTML]{C2E6CB}0.06  & \cellcolor[HTML]{F8696B}-0.19 & \cellcolor[HTML]{F7FCF8}0.01  & \cellcolor[HTML]{FEECED}-0.02 & \cellcolor[HTML]{EFF9F2}0.02  & \cellcolor[HTML]{FDFFFE}0.00  & \cellcolor[HTML]{FEF4F4}-0.01 & \cellcolor[HTML]{FEFDFD}0.00  & \cellcolor[HTML]{B9E2C4}0.07  & \cellcolor[HTML]{FEFCFC}0.00  & \cellcolor[HTML]{FEF3F3}-0.01 & \cellcolor[HTML]{FEFAFA}0.00  \\
… -\textgreater "…"              & \cellcolor[HTML]{E2F3E7}0.03  & \cellcolor[HTML]{F5FBF6}0.01  & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{F4FBF5}0.01  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{D4EDDB}0.04  & \cellcolor[HTML]{F98E90}-0.11 & \cellcolor[HTML]{FCCECE}-0.05 & \cellcolor[HTML]{C2E6CC}0.06  & \cellcolor[HTML]{FDD8D9}-0.04 & \cellcolor[HTML]{C1E6CB}0.06  & \cellcolor[HTML]{DBF0E1}0.03  & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{D4EEDB}0.04  & \cellcolor[HTML]{F8FDFA}0.01  & \cellcolor[HTML]{FDFEFD}0.00  \\
… -\textgreater '…'              & \cellcolor[HTML]{E4F4E9}0.03  & \cellcolor[HTML]{D7EFDD}0.04  & \cellcolor[HTML]{FEF4F4}-0.01 & \cellcolor[HTML]{D2ECD9}0.04  & \cellcolor[HTML]{FEF5F5}-0.01 & \cellcolor[HTML]{6AC181}0.14  & \cellcolor[HTML]{FCBFC0}-0.06 & \cellcolor[HTML]{FEFAFA}0.00  & \cellcolor[HTML]{95D3A5}0.10  & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{D3EDDA}0.04  & \cellcolor[HTML]{ECF7EF}0.02  & \cellcolor[HTML]{DDF1E2}0.03  & \cellcolor[HTML]{ECF7EF}0.02  & \cellcolor[HTML]{CFEBD7}0.05  & \cellcolor[HTML]{FEFFFE}0.00  \\
Q:                               & \cellcolor[HTML]{FAA1A2}-0.09 & \cellcolor[HTML]{F8696B}-0.30 & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{F8696B}-0.56 & \cellcolor[HTML]{FEF9F9}-0.01 & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FEFEFE}0.00  & \cellcolor[HTML]{DAF0E0}0.04  & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{FEF9F9}-0.01 & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{F8696B}-0.34 & \cellcolor[HTML]{F8696B}-0.20 & \cellcolor[HTML]{F8696B}-0.29 & \cellcolor[HTML]{FEF3F3}-0.01 & \cellcolor[HTML]{F8696B}-0.61 \\
these                            & \cellcolor[HTML]{A6DAB4}0.09  & \cellcolor[HTML]{FEEDED}-0.02 & \cellcolor[HTML]{63BE7B}0.18  & \cellcolor[HTML]{FBAFB0}-0.08 & \cellcolor[HTML]{F1F9F3}0.01  & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{85CC98}0.12  & \cellcolor[HTML]{FDE5E5}-0.03 & \cellcolor[HTML]{95D3A6}0.10  & \cellcolor[HTML]{FCCDCD}-0.05 & \cellcolor[HTML]{BFE5C9}0.06  & \cellcolor[HTML]{A2D8B0}0.09  & \cellcolor[HTML]{9ED7AD}0.09  & \cellcolor[HTML]{FEEDED}-0.02 & \cellcolor[HTML]{FDE9E9}-0.02 & \cellcolor[HTML]{FDDDDD}-0.03 \\
more                             & \cellcolor[HTML]{D2EDD9}0.04  & \cellcolor[HTML]{FBFEFC}0.00  & \cellcolor[HTML]{A0D8AF}0.09  & \cellcolor[HTML]{E9F6ED}0.02  & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{D9F0DF}0.04  & \cellcolor[HTML]{9FD7AE}0.09  & \cellcolor[HTML]{AEDEBB}0.08  & \cellcolor[HTML]{F6FCF8}0.01  & \cellcolor[HTML]{FEEBEB}-0.02 & \cellcolor[HTML]{6EC384}0.14  & \cellcolor[HTML]{FBBDBE}-0.07 & \cellcolor[HTML]{FBB6B7}-0.07 & \cellcolor[HTML]{FEF5F5}-0.01 & \cellcolor[HTML]{FCCDCE}-0.05 \\
using                            & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FCC5C6}-0.06 & \cellcolor[HTML]{63BE7B}0.42  & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{74C589}0.13  & \cellcolor[HTML]{FEEBEC}-0.02 & \cellcolor[HTML]{FEF8F8}-0.01 & \cellcolor[HTML]{F8696B}-0.25 & \cellcolor[HTML]{F2FAF4}0.01  & \cellcolor[HTML]{ECF7EF}0.02  & \cellcolor[HTML]{ECF7EF}0.02  & \cellcolor[HTML]{95D3A5}0.10  & \cellcolor[HTML]{FDE5E5}-0.03 & \cellcolor[HTML]{B6E1C1}0.07  & \cellcolor[HTML]{F2FAF4}0.01  \\
create -\textgreater write       & \cellcolor[HTML]{FEFEFE}0.00  & \cellcolor[HTML]{FEEEEE}-0.02 & \cellcolor[HTML]{71C487}0.14  & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{DAF0E0}0.04  & \cellcolor[HTML]{E8F6EC}0.02  & \cellcolor[HTML]{FDE2E3}-0.03 & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{FDE6E6}-0.02 & \cellcolor[HTML]{C8E8D0}0.05  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{F5FBF6}0.01  & \cellcolor[HTML]{FBB2B3}-0.08 & \cellcolor[HTML]{7CC990}0.13  & \cellcolor[HTML]{FA9C9D}-0.10 & \cellcolor[HTML]{E9F6EC}0.02  \\
sentence -\textgreater statement & \cellcolor[HTML]{F0F9F3}0.01  & \cellcolor[HTML]{DCF1E1}0.03  & \cellcolor[HTML]{FEF2F2}-0.01 & \cellcolor[HTML]{EDF8F0}0.02  & \cellcolor[HTML]{E6F5EA}0.02  & \cellcolor[HTML]{FCC8C9}-0.05 & \cellcolor[HTML]{FAA1A2}-0.09 & \cellcolor[HTML]{FEFDFD}0.00  & \cellcolor[HTML]{E6F5EA}0.02  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FCFEFD}0.00  & \cellcolor[HTML]{F86C6E}-0.15 & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{FEF8F8}-0.01 & \cellcolor[HTML]{FCCECE}-0.05 & \cellcolor[HTML]{FDE6E6}-0.02 \\
create -\textgreater generate    & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{C1E5CB}0.06  & \cellcolor[HTML]{FEF4F4}-0.01 & \cellcolor[HTML]{FDE4E4}-0.03 & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{7BC88F}0.13  & \cellcolor[HTML]{FEE9EA}-0.02 & \cellcolor[HTML]{FDE6E7}-0.02 & \cellcolor[HTML]{FDE4E4}-0.03 & \cellcolor[HTML]{B7E1C2}0.07  & \cellcolor[HTML]{FEF3F3}-0.01 & \cellcolor[HTML]{FEEEEE}-0.02 & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{FEEBEC}-0.02 & \cellcolor[HTML]{C5E7CE}0.06  & \cellcolor[HTML]{F5FBF6}0.01  \\
compose -\textgreater write      & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{F0F9F2}0.02  & \cellcolor[HTML]{63BE7B}0.27  & \cellcolor[HTML]{FEEBEC}-0.02 & \cellcolor[HTML]{EBF7EE}0.02  & \cellcolor[HTML]{CEEBD6}0.05  & \cellcolor[HTML]{FDDEDE}-0.03 & \cellcolor[HTML]{FEFAFA}0.00  & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{63BE7B}0.18  & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{FEF8F8}-0.01 & \cellcolor[HTML]{CAE9D2}0.05  & \cellcolor[HTML]{63BE7B}0.18  & \cellcolor[HTML]{FEF1F1}-0.01 & \cellcolor[HTML]{F6FBF7}0.01  \\
produce -\textgreater write      & \cellcolor[HTML]{FEF4F5}-0.01 & \cellcolor[HTML]{F1F9F3}0.01  & \cellcolor[HTML]{B4E0BF}0.07  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FEF7F7}-0.01 & \cellcolor[HTML]{FEECEC}-0.02 & \cellcolor[HTML]{FEFEFE}0.00  & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{FEFCFC}0.00  & \cellcolor[HTML]{CDEAD4}0.05  & \cellcolor[HTML]{FDD7D7}-0.04 & \cellcolor[HTML]{FEEBEB}-0.02 & \cellcolor[HTML]{BCE4C7}0.06  & \cellcolor[HTML]{69C181}0.14  & \cellcolor[HTML]{F98788}-0.12 & \cellcolor[HTML]{F0F9F2}0.02  \\
appears -\textgreater comes      & \cellcolor[HTML]{FDDFDF}-0.03 & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{63BE7B}0.22  & \cellcolor[HTML]{6BC282}0.14  & \cellcolor[HTML]{EDF8F0}0.02  & \cellcolor[HTML]{DCF1E1}0.03  & \cellcolor[HTML]{F5FBF7}0.01  & \cellcolor[HTML]{FCD3D4}-0.04 & \cellcolor[HTML]{FEF7F7}-0.01 & \cellcolor[HTML]{FDD8D9}-0.04 & \cellcolor[HTML]{FDE2E2}-0.03 & \cellcolor[HTML]{91D1A2}0.11  & \cellcolor[HTML]{C3E6CC}0.06  & \cellcolor[HTML]{65BF7D}0.15  & \cellcolor[HTML]{83CB96}0.12  & \cellcolor[HTML]{63BE7B}0.17  \\
and -\textgreater or             & \cellcolor[HTML]{F7FCF8}0.01  & \cellcolor[HTML]{E9F6EC}0.02  & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{F4FBF6}0.01  & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{FEEEEE}-0.02 & \cellcolor[HTML]{63BE7B}0.23  & \cellcolor[HTML]{74C58A}0.13  & \cellcolor[HTML]{9BD6AB}0.10  & \cellcolor[HTML]{E3F4E8}0.03  & \cellcolor[HTML]{FDDDDD}-0.03 & \cellcolor[HTML]{FDE7E7}-0.02 & \cellcolor[HTML]{E4F4E8}0.03  & \cellcolor[HTML]{D9EFDF}0.04  & \cellcolor[HTML]{FEEDED}-0.02 & \cellcolor[HTML]{EBF7EE}0.02  \\
a -\textgreater the              & \cellcolor[HTML]{FEFCFC}0.00  & \cellcolor[HTML]{F0F9F3}0.01  & \cellcolor[HTML]{EFF9F2}0.02  & \cellcolor[HTML]{68C07F}0.15  & \cellcolor[HTML]{F7FCF9}0.01  & \cellcolor[HTML]{EEF8F1}0.02  & \cellcolor[HTML]{DCF1E1}0.03  & \cellcolor[HTML]{FBFEFC}0.00  & \cellcolor[HTML]{E3F3E7}0.03  & \cellcolor[HTML]{FDE5E5}-0.03 & \cellcolor[HTML]{D9F0DF}0.04  & \cellcolor[HTML]{FEE9EA}-0.02 & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{D2EDD9}0.04  & \cellcolor[HTML]{E7F5EB}0.02  & \cellcolor[HTML]{FBFEFC}0.00  \\
lesser -\textgreater smaller     & \cellcolor[HTML]{F5FBF7}0.01  & \cellcolor[HTML]{F7FCF8}0.01  & \cellcolor[HTML]{FEF3F3}-0.01 & \cellcolor[HTML]{63BE7B}0.17  & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{FEEEEE}-0.02 & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{FEECEC}-0.02 & \cellcolor[HTML]{FDD8D9}-0.04 & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{FEEBEB}-0.02 & \cellcolor[HTML]{F0F9F2}0.02  & \cellcolor[HTML]{AEDEBB}0.08  & \cellcolor[HTML]{FEECEC}-0.02 & \cellcolor[HTML]{FEFFFE}0.00  & \cellcolor[HTML]{FEECEC}-0.02 \\
generate -\textgreater provide   & \cellcolor[HTML]{F98B8D}-0.12 & \cellcolor[HTML]{FCC0C1}-0.06 & \cellcolor[HTML]{F2FAF4}0.01  & \cellcolor[HTML]{F4FBF5}0.01  & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{F98E90}-0.11 & \cellcolor[HTML]{F9FDFA}0.01  & \cellcolor[HTML]{E8F6EB}0.02  & \cellcolor[HTML]{E8F6EB}0.02  & \cellcolor[HTML]{70C486}0.14  & \cellcolor[HTML]{EDF8F0}0.02  & \cellcolor[HTML]{EDF8F0}0.02  & \cellcolor[HTML]{FEF0F0}-0.01 & \cellcolor[HTML]{FEEBEC}-0.02 & \cellcolor[HTML]{FBFDFB}0.00  & \cellcolor[HTML]{FBB1B2}-0.08 \\
excludes -\textgreater omits     & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{9CD6AB}0.10  & \cellcolor[HTML]{FBABAC}-0.08 & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{D8EFDE}0.04  & \cellcolor[HTML]{7AC88F}0.13  & \cellcolor[HTML]{FEF2F2}-0.01 & \cellcolor[HTML]{FEF8F8}-0.01 & \cellcolor[HTML]{63BE7B}0.16  & \cellcolor[HTML]{F2FAF4}0.01  & \cellcolor[HTML]{DEF2E3}0.03  & \cellcolor[HTML]{7AC88F}0.13  & \cellcolor[HTML]{63BE7B}0.21  & \cellcolor[HTML]{FEEBEC}-0.02 & \cellcolor[HTML]{FEF8F8}-0.01 \\
excludes -\textgreater lacks     & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{B7E1C2}0.07  & \cellcolor[HTML]{67C07E}0.15  & \cellcolor[HTML]{FEFBFB}0.00  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{A1D8B0}0.09  & \cellcolor[HTML]{80CA94}0.12  & \cellcolor[HTML]{FDD8D9}-0.04 & \cellcolor[HTML]{F8696B}-0.28 & \cellcolor[HTML]{63BE7B}0.46  & \cellcolor[HTML]{FEF8F8}-0.01 & \cellcolor[HTML]{E6F5EA}0.02  & \cellcolor[HTML]{FBBCBD}-0.07 & \cellcolor[HTML]{C5E7CE}0.06  & \cellcolor[HTML]{FBB9BA}-0.07 & \cellcolor[HTML]{FEF1F1}-0.01 \\
lacks -\textgreater omits        & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{D0ECD7}0.05  & \cellcolor[HTML]{F8696B}-0.18 & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{F99394}-0.11 & \cellcolor[HTML]{DFF2E4}0.03  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{D8EFDE}0.04  & \cellcolor[HTML]{F8696B}-0.22 & \cellcolor[HTML]{F0F9F2}0.02  & \cellcolor[HTML]{FDE7E8}-0.02 & \cellcolor[HTML]{63BE7B}0.27  & \cellcolor[HTML]{63BE7B}0.32  & \cellcolor[HTML]{B8E2C3}0.07  & \cellcolor[HTML]{FEEFEF}-0.02 \\
contain -\textgreater have       & \cellcolor[HTML]{FEEDEE}-0.02 & \cellcolor[HTML]{FEEDEE}-0.02 & \cellcolor[HTML]{F8696B}-0.32 & \cellcolor[HTML]{F7FCF8}0.01  & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FBFEFC}0.00  & \cellcolor[HTML]{DCF1E1}0.03  & \cellcolor[HTML]{FDDCDD}-0.03 & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{90D1A1}0.11  & \cellcolor[HTML]{C6E7CF}0.06  & \cellcolor[HTML]{FCCBCC}-0.05 & \cellcolor[HTML]{95D3A5}0.10  & \cellcolor[HTML]{FEF2F2}-0.01 & \cellcolor[HTML]{F2FAF4}0.01  & \cellcolor[HTML]{FEF6F6}-0.01 \\
have -\textgreater include       & \cellcolor[HTML]{FAA2A3}-0.09 & \cellcolor[HTML]{F99394}-0.11 & \cellcolor[HTML]{63BE7B}0.45  & \cellcolor[HTML]{FEF7F7}-0.01 & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{FDD8D9}-0.04 & \cellcolor[HTML]{FDE7E8}-0.02 & \cellcolor[HTML]{FFFFFF}0.00  & \cellcolor[HTML]{78C78C}0.13  & \cellcolor[HTML]{F99394}-0.11 & \cellcolor[HTML]{FCD0D1}-0.05 & \cellcolor[HTML]{F0F9F2}0.02  & \cellcolor[HTML]{D0ECD7}0.05  & \cellcolor[HTML]{63BE7B}0.25  & \cellcolor[HTML]{FEF7F7}-0.01 & \cellcolor[HTML]{FFFFFF}0.00 
\end{tabular}%
}
\caption{
\madd{Average performance differences between various models for the most common minimal edits to instruction templates in the \lmentry{} benchmark (e.g., substituting `excludes' with `lacks'). The `count' column indicates the number of template pairs affected by each edit.} \gabis{(1) this figure is actually a table, can we remake it with latex tables? (2) The two first columns are missing headers, the first column can be removed I think, the second one should have a title, maybe ``Edit''? (3) What do we mean by ``most common'' in what sense are they most common? Maybe we can omit the count column (4) font is too small, maybe remove some models.}
}\label{tab:edit_dist_pairs}
\end{table}

==> tables/openai_avg_default.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc} \toprule
                                   & \multicolumn{1}{c}{\textbf{davinci}} & \multicolumn{1}{c}{\textbf{td002}} & \multicolumn{1}{c}{\textbf{td003}} & \multicolumn{1}{c}{\textbf{cgpt}} \\ \hline
\textbf{all words from   category} & 0.56                                 & 0.72                               & 0.84                               & 0.60                              \\
\textbf{any words from   category} & 0.55                                 & 0.63                               & 0.65                               & 0.86                              \\
\textbf{ends with word}            & 0.10                                 & 0.30                               & 0.58                               & 0.60                              \\
\textbf{first   alphabetically}    & 0.46                                 & 0.48                               & 0.71                               & 0.98                              \\
\textbf{homophones}                & 0.48                                 & 0.19                               & 0.38                               & 0.49                              \\
\textbf{less letters}              & 0.41                                 & 0.67                               & 0.79                               & 0.88                              \\
\textbf{more letters}              & 0.47                                 & 0.68                               & 0.82                               & 0.87                              \\
\textbf{rhyming word}              & 0.19                                 & 0.29                               & 0.57                               & 0.69                              \\
\textbf{word before}               & 0.12                                 & 0.13                               & 0.27                               & 0.40                              \\
\textbf{word not   containing}     & 0.03                                 & 0.85                               & 0.97                               & 0.90      \\ \bottomrule                       
\end{tabular}%
}
\caption{
 Average performances for OpenAI models across all \lmentry{} tasks, computed using only the original prompts.
 }
\label{tab:openai_avg_deafult}
\end{table}

==> tables/openai_avg_perdicted_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc} \toprule
                                   & \multicolumn{1}{c}{\textbf{davinci}} & \multicolumn{1}{c}{\textbf{td002}} & \multicolumn{1}{c}{\textbf{td003}} & \multicolumn{1}{c}{\textbf{cgpt}} \\ \hline
\textbf{all words from   category} & 0.15                                 & 0.61                               & 0.79                               & 0.62                              \\
\textbf{any words from   category} & 0.16                                 & 0.62                               & 0.59                               & 0.82                              \\
\textbf{ends with word}            & 0.11                                 & 0.24                               & 0.42                               & 0.54                              \\
\textbf{first   alphabetically}    & 0.12                                 & 0.27                               & 0.35                               & 0.45                              \\
\textbf{homophones}                & 0.12                                 & 0.57                               & 0.60                               & 0.71                              \\
\textbf{less letters}              & 0.17                                 & 0.51                               & 0.58                               & 0.58                              \\
\textbf{more letters}              & 0.16                                 & 0.49                               & 0.51                               & 0.50                              \\
\textbf{rhyming word}              & 0.14                                 & 0.39                               & 0.41                               & 0.76                              \\
\textbf{word before}               & 0.04                                 & 0.16                               & 0.51                               & 0.47                              \\
\textbf{word not   containing}     & 0.06                                 & 0.57                               & 0.84                               & 0.81      \\ \bottomrule                       
\end{tabular}%
}
\caption{Estimated average performances for OpenAI models across all \lmentry{} tasks, approximated using all prompt paraphrases.}
\label{tab:openai_avg_all}
\end{table}

==> tables/openai_avg_repetitions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[!htbp]
\begin{adjustwidth}{-1cm}{-1cm}
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{l|cccccccccccccccc}
\toprule
\textbf{task}                      & \textbf{t0\_3b} & \textbf{t0++} & \textbf{fal7b} & \textbf{mpt7b} & \textbf{alp7b} & \textbf{alp13b} & \textbf{ft5small} & \textbf{ft5base} & \textbf{ft5large} & \textbf{ft5xl} & \textbf{ft5xxl} & \textbf{airoboros} & \textbf{noushermes} & \textbf{ultralm} & \textbf{vicuna} & \textbf{minotaur} \\ \hline
\textbf{all words from   category} & 4.9             & 2.2           & 11.3               & 4.2             & 3.1                & 2.9                 & 5.6                    & 4.3                   & 2.4                    & 6.6                 & 3.1                  & 6.6                    & 8.7                      & 3.2                  & 3.8                 & 7.5                   \\
\textbf{any words from   category} & 3.4             & 1.5           & 11.2               & 4.1             & 3.8                & 2.9                 & 11                     & 7.3                   & 6.7                    & 2                   & 1.7                  & 5.8                    & 3.2                      & 6                    & 2.6                 & 2.1                   \\
\textbf{ends with word}            & 3.3             & 4.3           & 2.2                & 2.4             & 1.9                & 10.7                & 3.3                    & 6.2                   & 5.7                    & 5.9                 & 6.1                  & 2.8                    & 3.5                      & 2                    & 3.7                 & 2.5                   \\
\textbf{first   alphabetically}    & 10.3            & 3.2           & 7.2                & 6.1             & 2.6                & 6.4                 & 10.3                   & 3.2                   & 5.1                    & 3.9                 & 4                    & 5.3                    & 8.2                      & 11.4                 & 5.7                 & 7.8                   \\
\textbf{homophones}                & 7.2             & 5.7           & 8.3                & 10.3            & 2.4                & 4.2                 & 10.5                   & 4.5                   & 3.5                    & 3.7                 & 9.7                  & 5.8                    & 10.8                     & 2.1                  & 3.7                 & 1.2                   \\
\textbf{less letters}              & 3.3             & 9.5           & 5.3                & 3.8             & 4.2                & 5.5                 & 5.9                    & 4.6                   & 4.5                    & 5.1                 & 3.5                  & 4.2                    & 3.5                      & 7.1                  & 10.2                & 6.3                   \\
\textbf{more letters}              & 4.3             & 4.2           & 6.5                & 6               & 5.8                & 10.4                & 3.3                    & 4.2                   & 4.2                    & 4.9                 & 7.6                  & 5.4                    & 9.3                      & 6                    & 7.9                 & 6.8                   \\
\textbf{rhyming word}              & 10.9            & 2.5           & 4.1                & 5.2             & 2.6                & 12.8                & 6.6                    & 3.8                   & 6.7                    & 5.1                 & 5.6                  & 3.3                    & 3.8                      & 1.8                  & 7.3                 & 1.2                   \\
\textbf{word before}               & 5.9             & 2.8           & 1.3                & 3.2             & 6.6                & 3.5                 & 6                      & 4.4                   & 4.5                    & 8.8                 & 4.9                  & 4.5                    & 3.3                      & 1.1                  & 5.1                 & 2                     \\
\textbf{word not   containing}     & 4.2             & 12.4          & 8.6                & 11.8            & 9.4                & 6.3                 & 4.4                    & 10                    & 21.9                   & 14.2                & 5.8                  & 10.1                   & 5.8                      & 6.3                  & 5                   & 12.3 \\ \bottomrule                
\end{tabular}%
}
\caption{The average number of average heuristic repetitions required to achieve less than a 1 accuracy point discrepancy from the actual average performance for each task and open-source model. Maximal value: 21.9. All values average: 5.62 (std: 3.12).}
\label{tab:openai_avg_repetitions}
\end{adjustwidth}
\end{table*}

==> tables/openai_max_default.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc} \toprule
                                   & \multicolumn{1}{c}{\textbf{davinci}} & \multicolumn{1}{c}{\textbf{td002}} & \multicolumn{1}{c}{\textbf{td003}} & \multicolumn{1}{c}{\textbf{cgpt}} \\ \hline
\textbf{all words from   category} & 0.64                                 & 0.80                               & 0.85                               & 0.68                              \\
\textbf{any words from   category} & 0.66                                 & 0.82                               & 0.88                               & 0.97                              \\
\textbf{ends with word}            & 0.15                                 & 0.35                               & 0.61                               & 0.62                              \\
\textbf{first   alphabetically}    & 0.50                                 & 0.56                               & 0.90                               & 0.98                              \\
\textbf{homophones}                & 0.59                                 & 0.25                               & 0.41                               & 0.79                              \\
\textbf{less letters}              & 0.48                                 & 0.70                               & 0.86                               & 0.92                              \\
\textbf{more letters}              & 0.54                                 & 0.80                               & 0.89                               & 0.90                              \\
\textbf{rhyming word}              & 0.32                                 & 0.45                               & 0.65                               & 0.96                              \\
\textbf{word before}               & 0.17                                 & 0.21                               & 0.34                               & 0.66                              \\
\textbf{word not   containing}     & 0.04                                 & 0.92                               & 1.00                               & 0.96      \\ \bottomrule                       
\end{tabular}%
}
\caption{Max performances for OpenAI models across all \lmentry{} tasks, computed using only the original prompts.}
\label{tab:openai_max_default}
\end{table}

==> tables/openai_max_heuristic.tex <==
%Generate Result (click "Generate" to refresh) Copy to clipboard
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[!htbp]
\begin{adjustwidth}{-1cm}{-1cm}
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{l|cccccccccccccccc}
\toprule
\textbf{task}                      & \textbf{t0\_3b} & \textbf{t0++} & \textbf{fal7b} & \textbf{mpt7b} & \textbf{alp7b} & \textbf{alp13b} & \textbf{ft5small} & \textbf{ft5base} & \textbf{ft5large} & \textbf{ft5xl} & \textbf{ft5xxl} & \textbf{airoboros} & \textbf{noushermes} & \textbf{ultralm} & \textbf{vicuna} & \textbf{minotaur} \\ \hline
\textbf{all words from   category} & \checkmark{}              & \checkmark{}            & 0.01           & \checkmark{}             & \checkmark{}             & \checkmark{}              & 0.03              & \checkmark{}               & 0.02              & \checkmark{}             & \checkmark{}              & \checkmark{}                 & 0.02                & \checkmark{}               & \checkmark{}              & \checkmark{}                \\
\textbf{any words from   category} & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & \checkmark{}                & \checkmark{}               & \checkmark{}                & \checkmark{}             & \checkmark{}              & \checkmark{}                 & 0.06                & \checkmark{}               & \checkmark{}              & \checkmark{}                \\
\textbf{ends with word}            & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & \checkmark{}                & \checkmark{}               & \checkmark{}                & \checkmark{}             & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & \checkmark{}              & 0.03              \\
\textbf{first   alphabetically}    & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & 0.01              & \checkmark{}               & 0.03              & 0.03           & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & \checkmark{}              & \checkmark{}                \\
\textbf{homophones}                & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & \checkmark{}                & \checkmark{}               & 0.04              & \checkmark{}             & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & \checkmark{}              & 0.01              \\
\textbf{less letters}              & \checkmark{}              & 0.02          & 0.01           & \checkmark{}             & \checkmark{}             & \checkmark{}              & 0.02              & \checkmark{}               & 0.03              & \checkmark{}             & 0.02            & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & \checkmark{}              & \checkmark{}                \\
\textbf{more letters}              & 0.01            & 0.01          & \checkmark{}             & 0.03           & \checkmark{}             & \checkmark{}              & \checkmark{}                & \checkmark{}               & \checkmark{}                & 0.01           & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & 0.01             & \checkmark{}              & \checkmark{}                \\
\textbf{rhyming word}              & \checkmark{}              & 0.01          & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & 0.02              & 0.03             & 0.01              & 0.01           & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & 0.01             & \checkmark{}              & \checkmark{}                \\
\textbf{word before}               & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & 0.01           & \checkmark{}              & \checkmark{}                & \checkmark{}               & \checkmark{}                & \checkmark{}             & 0.06            & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & 0.01            & \checkmark{}                \\
\textbf{word not   containing}     & \checkmark{}              & \checkmark{}            & \checkmark{}             & \checkmark{}             & \checkmark{}             & \checkmark{}              & \checkmark{}                & \checkmark{}               & \checkmark{}                & \checkmark{}             & \checkmark{}              & \checkmark{}                 & \checkmark{}                  & \checkmark{}               & \checkmark{}              & \checkmark{}    \\ \hline           
\end{tabular}%
}
\caption{Results of the greedy optimal paraphrase search for each task and open-source model. An optimal prompt was recovered in 130 out of 160 cases. In the remaining cases, the average discrepancy in performance between the chosen and actual optimal paraphrases was 2.1 accuracy points, with a standard deviation of 1.4.}
\label{tab:openai_max_heuristic}
\end{adjustwidth}
\end{table*}

==> tables/openai_max_predicted_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc} \toprule
                                   & \multicolumn{1}{c}{\textbf{davinci}} & \multicolumn{1}{c}{\textbf{td002}} & \multicolumn{1}{c}{\textbf{td003}} & \multicolumn{1}{c}{\textbf{cgpt}} \\ \hline
\textbf{all words from   category} & 0.64                                 & 0.94                               & 0.99                               & 0.97                              \\
\textbf{any words from   category} & 0.66                                 & 0.95                               & 0.99                               & 1.00                              \\
\textbf{ends with word}            & 0.88                                 & 0.52                               & 0.67                               & 0.72                              \\
\textbf{first   alphabetically}    & 0.55                                 & 0.95                               & 0.97                               & 1.00                              \\
\textbf{homophones}                & 0.63                                 & 0.99                               & 0.95                               & 0.99                              \\
\textbf{less letters}              & 0.61                                 & 0.95                               & 0.95                               & 1.00                              \\
\textbf{more letters}              & 0.71                                 & 0.93                               & 0.97                               & 1.00                              \\
\textbf{rhyming word}              & 0.67                                 & 0.93                               & 0.95                               & 0.99                              \\
\textbf{word before}               & 0.26                                 & 0.51                               & 0.82                               & 0.95                              \\
\textbf{word not   containing}     & 0.65                                 & 1.00                               & 1.00                               & 1.00   \\ \bottomrule                          
\end{tabular}%
}
\caption{Estimated max performances for OpenAI models across all \lmentry{} tasks, approximated using all prompt paraphrases.}
\label{tab:openai_max_all}
\end{table}

==> tables/openai_mcnemar_test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder\underline{ine}\underline{}{}
\begin{table}[!htbp]
\begin{adjustwidth}{-0.5cm}{0cm}
\resizebox{1.05\columnwidth}{!}{%
\begin{tabular}{lcccc} \toprule
\textbf{task}                      & \textbf{davinci}        & \textbf{td002}          & \textbf{td003}          & \textbf{cgpt}           \\ \hline
\textbf{all words from   category} & 1                       & \underline{{.0009}} & \underline{{.0002}} & \underline{{7.2E-08}} \\
\textbf{any words from category} & 1                       & \underline{{.0008}} & \underline{{.0009}} & .0832                \\
\textbf{ends with word}            & \underline{{8.8E-17}} & \underline{{.0195}} & .3034                & .0955                \\
\textbf{first   alphabetically}    & .4922                & \underline{{6.1E-09}} & \underline{{.0196}} & .1572                \\
\textbf{homophones}                & .5371               & \underline{{7.8E-18}} & \underline{{5.3E-13}} & \underline{{7.7E-06}} \\
\textbf{less letters}              & .0633                & \underline{{3.4E-06}} & \underline{{.0009}} & \underline{{.0047}} \\
\textbf{more letters}              & \underline{{.0131}} & \underline{{.0046}} & \underline{{.0209}} & \underline{{.0016}} \\
\textbf{rhyming word}              & \underline{{5.7E-07}} & \underline{{1.4E-10}} & \underline{{4.3E-08}} & .0833                \\
\textbf{word before}               & .10560                & \underline{{1.1E-06}} & \underline{{1.1E-11}} & \underline{{1.9E-06}} \\
\textbf{word not containing}       & \underline{{6.3E-05}} & .1573                & 1                       & .3173 \\ \bottomrule               
\end{tabular}
}\caption{
The results for the McNemar test we ran to assess the statistical significance of the differences in maximum performance between the original best prompt and the prompt estimated to be optimal across all paraphrases for each task in the \lmentry{} benchmark. Significant max differences (p-value<0.05) are highlighted. 
}
\label{tab:openai_mecnemar}
\end{adjustwidth}
\end{table}

==> tables/optimal_sources_bbh.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
\textbf{model}                                  & \textbf{default}                     & \textbf{rephrase}                     & \textbf{cot}                          & \textbf{gradual}                      \\ \hline
\textbf{falcon-7b}                              & 0.00                                 & 27.27                                 & 18.18                                 & \textbf{54.55}                        \\
\textbf{mpt-7b}                                 & 0.00                                 & 40.00                                 & 16.00                                 & \textbf{44.00}                        \\
\textbf{flan-t5-xl}                             & 2.38                                 & 23.81                                 & 26.19                                 & \textbf{47.62}                        \\
\textbf{flan-t5-xxl}                            & 4.35                                 & 17.39                                 & 26.09                                 & \textbf{52.17}                        \\
\textbf{t0++}                                   & 0.00                                 & \textbf{50.00}                        & 40.00                                 & 10.00                                 \\
\textbf{alpaca-13b}                             & 0.00                                 & 11.11                                 & \textbf{44.44}                        & \textbf{44.44}                        \\
\textbf{airoboros-13b}                          & 0.00                                 & \textbf{50.00}                        & 16.67                                 & 33.33                                 \\
\textbf{nous-hermes-13b}                        & 0.00                                 & 12.50                                 & 16.67                                 & \textbf{70.83}                        \\
\textbf{ultralm-13b}                            & 0.00                                 & 29.17                                 & 25.00                                 & \textbf{45.83}                        \\
\textbf{vicuna-13b}                             & 0.00                                 & \textbf{38.10}                        & 28.57                                 & 33.33                                 \\
\textbf{minotaur-15b}                           & 0.00                                 & 9.09                                  & 0.00                                  & \textbf{90.91}                        \\ \hline
{\color[HTML]{4472C4} \textbf{all tasks}}       & {\color[HTML]{4472C4} \textbf{0.73}} & {\color[HTML]{4472C4} \textbf{27.37}} & {\color[HTML]{4472C4} \textbf{23.72}} & {\color[HTML]{4472C4} \textbf{48.18}} \\
{\color[HTML]{00B050} \textbf{all paraphrases}} & {\color[HTML]{00B050} \textbf{0.57}} & {\color[HTML]{00B050} \textbf{28.07}} & {\color[HTML]{00B050} \textbf{29.64}} & {\color[HTML]{00B050} \textbf{41.72}} \\ \bottomrule
\end{tabular}%
}
\caption{Distribution of optimal paraphrase sources per model for \bbh{}. Rows represent models and columns indicate paraphrase generation methods. Percentages in each cell show the rate of optimal paraphrases from each method, with bold numbers identifying the leading source for each model. The `All Models' row aggregates percentages across all models, while the `All Paraphrases' row displays the overall distribution of generation methods across all paraphrases.}
\label{tab:optimal_sources_bbh}
\end{table}

==> tables/optimal_sources_lmentry.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{model}                                  & \textbf{default}                     & \textbf{rephrase}                     & \textbf{cot}                          & \textbf{gradual}                      \\ \hline
\textbf{t0\_3b   (*)}                           & 0.00                                 & 11.76                                 & \textbf{58.82}                        & 29.41                                 \\
\textbf{t0++ (*)}                               & 0.00                                 & 15.00                                 & \textbf{45.00}                        & 40.00                                 \\
\textbf{falcon-7b}                              & 9.09                                 & 9.09                                  & 36.36                                 & \textbf{45.45}                        \\
\textbf{mpt-7b}                                 & 0.00                                 & 23.53                                 & \textbf{47.06}                        & 29.41                                 \\
\textbf{alpaca-7b (**)}                         & 8.33                                 & 0.00                                  & 0.00                                  & \textbf{91.67}                        \\
\textbf{alpaca-13b (**)}                        & 0.00                                 & 0.00                                  & 8.33                                  & \textbf{91.67}                        \\
\textbf{flan-t5-base (*)}                       & 0.00                                 & 7.14                                  & \textbf{64.29}                        & 28.57                                 \\
\textbf{flan-t5-small (*)}                      & 0.00                                 & 0.00                                  & \textbf{58.33}                        & 41.67                                 \\
\textbf{flan-t5-large (*)}                      & 0.00                                 & \textbf{40.00}                        & \textbf{40.00}                        & 20.00                                 \\
\textbf{flan-t5-xl (*)}                         & 0.00                                 & 7.69                                  & 30.77                                 & \textbf{61.54}                        \\
\textbf{flan-t5-xxl (*)}                        & 0.00                                 & 13.04                                 & \textbf{69.57}                        & 17.39                                 \\
\textbf{airoboros-13b (**)}                     & 0.00                                 & 35.71                                 & 14.29                                 & \textbf{50.00}                        \\
\textbf{nous-hermes-13b   (**)}                 & 0.00                                 & 0.00                                  & 33.33                                 & \textbf{66.67}                        \\
\textbf{ultralm-13b (**)}                       & 0.00                                 & 6.67                                  & \textbf{66.67}                        & 26.67                                 \\
\textbf{vicuna-13b (**)}                        & 10.00                                & 10.00                                 & 0.00                                  & \textbf{80.00}                        \\
\textbf{minotaur-15b}                           & 0.00                                 & 14.29                                 & 28.57                                 & \textbf{57.14}                        \\ \hline
{\color[HTML]{4472C4} \textbf{all models}}      & {\color[HTML]{0070C0} \textbf{1.33}} & {\color[HTML]{0070C0} \textbf{12.39}} & {\color[HTML]{0070C0} \textbf{40.71}} & {\color[HTML]{0070C0} \textbf{45.58}} \\
{\color[HTML]{00B050} \textbf{all paraphrases}} & {\color[HTML]{00B050} \textbf{1.24}} & {\color[HTML]{00B050} \textbf{18.98}} & {\color[HTML]{00B050} \textbf{52.94}} & {\color[HTML]{00B050} \textbf{26.84}} \\ \bottomrule
\end{tabular}%
}
\caption{Distribution of optimal paraphrase sources per model for \lmentry{}. Rows represent models, with T5-based models marked by an asterisk (*) and \llama{}-based models by two asterisks (**). Columns indicate paraphrase generation methods. Percentages in each cell show the rate of optimal paraphrases from each method, with bold numbers identifying the leading source for each model. The `All Models' row aggregates percentages across all models, while the `All Paraphrases' row displays the overall distribution of generation methods across all paraphrases.}
\label{tab:optimal_sources_lmentry}
\end{table}

==> tables/paraphrases_correctness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[bt!]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lccccc}
\toprule
\textbf{Benchmark \& Task}          & \textbf{Method}                                                        & \textbf{\begin{tabular}[c]{@{}c@{}}\#Auto \\ Paraphrases\end{tabular}}                                     & \textbf{\begin{tabular}[c]{@{}c@{}}\#Correct \\ Paraphrases\end{tabular}}                                  & \textbf{\begin{tabular}[c]{@{}l@{}}Correct \\ Ratio (\%)\end{tabular}}                                                   & \textbf{\begin{tabular}[c]{@{}l@{}}Model\\ Accuracy \\ (Avg.)\end{tabular}}                                & \textbf{\begin{tabular}[c]{@{}l@{}}Model\\ Accuracy \\ (Std.)\end{tabular}}                               \\
\hline
 all words from category             & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}258\\ 48\\ 133\\ 74\end{tabular}     & \begin{tabular}[c]{@{}l@{}}227\\ 39\\ 131\\ 54\end{tabular}     & \begin{tabular}[c]{@{}l@{}}87.98\%\\ 81.25\%\\ 98.50\%\\ 72.97\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.519\\ .483\\ .494\\ .604\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.074\\ .035\\ .065\\ .048\end{tabular} \\ \midrule
any words from category             & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}259\\ 48\\ 135\\ 72\end{tabular}     & \begin{tabular}[c]{@{}l@{}}233\\ 44\\ 134\\ 52\end{tabular}     & \begin{tabular}[c]{@{}l@{}}89.96\%\\ 91.67\%\\ 99.26\%\\ 71.23\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.443\\ .451\\ .438\\ .444\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.083\\ .043\\ .034\\ .160\end{tabular} \\ \midrule
ends with word                      & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}226\\ 47\\ 129\\ 47\end{tabular}     & \begin{tabular}[c]{@{}l@{}}210\\ 39\\ 126\\ 42\end{tabular}     & \begin{tabular}[c]{@{}l@{}}92.92\%\\ 82.98\%\\ 97.67\%\\ 89.36\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.131\\ .130\\ .138\\ .112\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.024\\ .022\\ .019\\ .027\end{tabular} \\ \midrule
first alphabetically                & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}233\\ 47\\ 121\\ 62\end{tabular}     & \begin{tabular}[c]{@{}l@{}}198\\ 38\\ 117\\ 40\end{tabular}     & \begin{tabular}[c]{@{}l@{}}84.98\%\\ 80.85\%\\ 96.69\%\\ 64.52\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.326\\ .293\\ .315\\ .381\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.079\\ .080\\ .076\\ .053\end{tabular} \\ \midrule
homophones                          & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}264\\ 48\\ 140\\ 73\end{tabular}     & \begin{tabular}[c]{@{}l@{}}234\\ 43\\ 128\\ 60\end{tabular}     & \begin{tabular}[c]{@{}l@{}}88.64\%\\ 89.58\%\\ 91.43\%\\ 82.19\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.252\\ .214\\ .246\\ .292\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.057\\ .023\\ .037\\ .081\end{tabular} \\ \midrule
less letters                        & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}240\\ 42\\ 126\\ 69\end{tabular}     & \begin{tabular}[c]{@{}l@{}}207\\ 40\\ 119\\ 45\end{tabular}     & \begin{tabular}[c]{@{}l@{}}86.25\%\\ 95.24\%\\ 94.44\%\\ 65.22\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.338\\ .316\\ .319\\ .397\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.078\\ .061\\ .068\\ .074\end{tabular} \\ \midrule
more letters                        & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}237\\ 45\\ 127\\ 62\end{tabular}     & \begin{tabular}[c]{@{}l@{}}210\\ 42\\ 123\\ 42\end{tabular}     & \begin{tabular}[c]{@{}l@{}}88.61\%\\ 93.33\%\\ 96.85\%\\ 67.74\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.374\\ .349\\ .359\\ .431\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.081\\ .059\\ .075\\ .078\end{tabular} \\ \midrule
rhyming word                        & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}245\\ 47\\ 125\\ 70\end{tabular}     & \begin{tabular}[c]{@{}l@{}}219\\ 37\\ 115\\ 64\end{tabular}     & \begin{tabular}[c]{@{}l@{}}89.39\%\\ 78.72\%\\ 92.00\%\\ 91.43\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.234\\ .189\\ .198\\ .325\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.079\\ .038\\ .049\\ .067\end{tabular} \\ \midrule
word before                         & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}233\\ 41\\ 125\\ 64\end{tabular}     & \begin{tabular}[c]{@{}l@{}}225\\ 39\\ 119\\ 64\end{tabular}     & \begin{tabular}[c]{@{}l@{}}96.57\%\\ 95.12\%\\ 95.20\%\\ 100.0\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.123\\ .088\\ .098\\ .195\end{tabular} & \begin{tabular}[c]{@{}l@{}}.049\\ .009\\ .012\\ .032\end{tabular} \\ \midrule
word not containing                 & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}234\\ 48\\ 125\\ 58\end{tabular}     & \begin{tabular}[c]{@{}l@{}}223\\ 47\\ 122\\ 51\end{tabular}     & \begin{tabular}[c]{@{}l@{}}95.30\%\\ 97.92\%\\ 97.60\%\\ 87.93\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.222\\ .177\\ .190\\ .337\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.094\\ .059\\ .043\\ .115\end{tabular} \\ \midrule
all tasks                           & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}2429\\ 461\\ 1286\\ 652\end{tabular} & \begin{tabular}[c]{@{}l@{}}2186\\ 408\\ 1234\\ 514\end{tabular} & \begin{tabular}[c]{@{}l@{}}90.00\%\\ 88.50\%\\ 95.96\%\\ 78.83\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.296\\ .269\\ .279\\ .351\end{tabular}   & \begin{tabular}[c]{@{}l@{}}.070\\ .043\\ .048\\ .074\end{tabular} \\ 
\bottomrule
\end{tabular}%
}
\caption{
The distribution of correct paraphrases for each generation method across all tasks in \lmentry{}.
}
\label{table:paraphrases_correctness_lmentry}
% \end{adjustwidth}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[tb!]
\begin{adjustwidth}{0.5cm}{0.5cm}
\small
\resizebox{0.92\textwidth}{!}{%
\begin{tabular}{l|lccccc}
\toprule
\textbf{Benchmark \& Task}          & \textbf{Method}                                                        & \textbf{\begin{tabular}[c]{@{}c@{}}\#Auto \\ Paraphrases\end{tabular}}                                     & \textbf{\begin{tabular}[c]{@{}c@{}}\#Correct \\ Paraphrases\end{tabular}}                                  & \textbf{\begin{tabular}[c]{@{}l@{}}Correct \\ Ratio (\%)\end{tabular}}                                                   & \textbf{\begin{tabular}[c]{@{}l@{}}Model\\ Accuracy \\ (Avg.)\end{tabular}}                                & \textbf{\begin{tabular}[c]{@{}l@{}}Model\\ Accuracy \\ (Std.)\end{tabular}}                               \\
\hline
causal judgement                    & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}187\\ 50\\ 60\\ 76\end{tabular}      & \begin{tabular}[c]{@{}l@{}}153\\ 31\\ 55\\ 66\end{tabular}      & \begin{tabular}[c]{@{}l@{}}81.82\%\\ 62.00\%\\ 91.67\%\\ 86.84\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.477\\ .469\\ .452\\ .502\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.034\\ .024\\ .023\\ .028\end{tabular} \\ \midrule
disambiguation qa                   & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}188\\ 50\\ 60\\ 77\end{tabular}      & \begin{tabular}[c]{@{}l@{}}177\\ 50\\ 50\\ 76\end{tabular}      & \begin{tabular}[c]{@{}l@{}}94.15\%\\ 100.0\%\\ 83.33\%\\ 98.70\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.412\\ .403\\ .357\\ .455\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.049\\ .031\\ .022\\ .029\end{tabular} \\ \midrule
formal fallacies                    & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}184\\ 50\\ 56\\ 77\end{tabular}      & \begin{tabular}[c]{@{}l@{}}130\\ 19\\ 51\\ 59\end{tabular}      & \begin{tabular}[c]{@{}l@{}}70.65\%\\ 38.00\%\\ 91.07\%\\ 76.62\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.308\\ .326\\ .294\\ .313\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.026\\ .027\\ .015\\ .027\end{tabular} \\ \midrule
geometric shapes                    & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}178\\ 50\\ 55\\ 72\end{tabular}      & \begin{tabular}[c]{@{}l@{}}171\\ 50\\ 53\\ 67\end{tabular}      & \begin{tabular}[c]{@{}l@{}}96.07\%\\ 100.0\%\\ 96.36\%\\ 93.06\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.163\\ .175\\ .153\\ .163\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.020\\ .015\\ .019\\ .020\end{tabular} \\ \midrule
hyperbaton                          & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}155\\ 43\\ 36\\ 75\end{tabular}      & \begin{tabular}[c]{@{}l@{}}117\\ 32\\ 35\\ 49\end{tabular}      & \begin{tabular}[c]{@{}l@{}}75.48\%\\ 74.42\%\\ 97.22\%\\ 65.33\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.466\\ .467\\ .438\\ .484\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.035\\ .020\\ .030\\ .034\end{tabular} \\ \midrule
logical deduction five objects      & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}189\\ 50\\ 59\\ 79\end{tabular}      & \begin{tabular}[c]{@{}l@{}}150\\ 47\\ 27\\ 75\end{tabular}      & \begin{tabular}[c]{@{}l@{}}79.37\%\\ 94.00\%\\ 45.76\%\\ 94.94\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.262\\ .239\\ .243\\ .283\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.027\\ .009\\ .026\\ .015\end{tabular} \\ \midrule
logical deduction seven objects     & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}186\\ 50\\ 60\\ 75\end{tabular}      & \begin{tabular}[c]{@{}l@{}}145\\ 41\\ 31\\ 72\end{tabular}      & \begin{tabular}[c]{@{}l@{}}77.96\%\\ 82.00\%\\ 51.67\%\\ 96.00\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.236\\ .215\\ .219\\ .257\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.026\\ .009\\ .028\\ .016\end{tabular} \\ \midrule
logical deduction three objects     & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}187\\ 50\\ 60\\ 76\end{tabular}      & \begin{tabular}[c]{@{}l@{}}147\\ 47\\ 27\\ 72\end{tabular}      & \begin{tabular}[c]{@{}l@{}}78.61\%\\ 94.00\%\\ 45.00\%\\ 94.74\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.359\\ .329\\ .317\\ .394\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.044\\ .023\\ .030\\ .028\end{tabular} \\ \midrule
movie recommendation                & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}180\\ 47\\ 57\\ 75\end{tabular}      & \begin{tabular}[c]{@{}l@{}}164\\ 47\\ 50\\ 66\end{tabular}      & \begin{tabular}[c]{@{}l@{}}91.11\%\\ 100.0\%\\ 87.72\%\\ 88.00\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.348\\ .371\\ .323\\ .351\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.036\\ .011\\ .040\\ .032\end{tabular} \\ \midrule
navigate                            & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}170\\ 50\\ 54\\ 65\end{tabular}      & \begin{tabular}[c]{@{}l@{}}152\\ 50\\ 54\\ 47\end{tabular}      & \begin{tabular}[c]{@{}l@{}}89.41\%\\ 100.0\%\\ 100.0\%\\ 72.31\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.386\\ .374\\ .388\\ .396\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.019\\ .013\\ .021\\ .017\end{tabular} \\ \midrule
penguins in a table                 & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}183\\ 49\\ 59\\ 74\end{tabular}      & \begin{tabular}[c]{@{}l@{}}143\\ 37\\ 51\\ 54\end{tabular}      & \begin{tabular}[c]{@{}l@{}}78.14\%\\ 75.51\%\\ 86.44\%\\ 72.97\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.243\\ .250\\ .215\\ .265\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.026\\ .014\\ .007\\ .018\end{tabular} \\ \midrule
ruin names                          & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}157\\ 50\\ 40\\ 66\end{tabular}      & \begin{tabular}[c]{@{}l@{}}143\\ 49\\ 35\\ 58\end{tabular}      & \begin{tabular}[c]{@{}l@{}}91.08\%\\ 98.00\%\\ 87.50\%\\ 87.88\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.254\\ .252\\ .250\\ .258\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.016\\ .015\\ .019\\ .013\end{tabular} \\ \midrule
salient translation error detection & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}136\\ 47\\ 25\\ 63\end{tabular}      & \begin{tabular}[c]{@{}l@{}}128\\ 46\\ 25\\ 56\end{tabular}      & \begin{tabular}[c]{@{}l@{}}94.12\%\\ 97.87\%\\ 100.0\%\\ 88.89\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.191\\ .185\\ .192\\ .196\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.015\\ .011\\ .007\\ .019\end{tabular} \\ \midrule
snarks                              & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}162\\ 50\\ 37\\ 74\end{tabular}      & \begin{tabular}[c]{@{}l@{}}152\\ 50\\ 37\\ 64\end{tabular}      & \begin{tabular}[c]{@{}l@{}}93.83\%\\ 100.0\%\\ 100.0\%\\ 86.49\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.405\\ .396\\ .410\\ .408\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.025\\ .024\\ .030\\ .021\end{tabular} \\ \midrule
sports understanding                & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}173\\ 48\\ 57\\ 67\end{tabular}      & \begin{tabular}[c]{@{}l@{}}137\\ 31\\ 49\\ 56\end{tabular}      & \begin{tabular}[c]{@{}l@{}}79.19\%\\ 64.58\%\\ 85.96\%\\ 83.58\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.461\\ .469\\ .453\\ .463\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.052\\ .051\\ .068\\ .035\end{tabular} \\ \midrule
all tasks                           & \begin{tabular}[c]{@{}l@{}}All\\ Rephrase\\ CoT\\ Gradual\end{tabular} & \begin{tabular}[c]{@{}l@{}}2615\\ 734\\ 775\\ 1091\end{tabular} & \begin{tabular}[c]{@{}l@{}}2209\\ 627\\ 630\\ 937\end{tabular}  & \begin{tabular}[c]{@{}l@{}}84.47\%\\ 85.42\%\\ 81.29\%\\ 85.88\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}.331\\ .327\\ .314\\ .346\end{tabular}  & \begin{tabular}[c]{@{}l@{}}.035\\ .025\\ .030\\ .029\end{tabular} \\
\bottomrule
\end{tabular}%

}
\caption{The distribution of correct paraphrases for each generation method across all tasks in \bbh{}.}
\label{table:paraphrases_correctness_bbh}
\end{adjustwidth}
\end{table*}






==> tables/tasks_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[bt!]
\begin{adjustwidth}{-1cm}{-1cm}
\small
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{lp{11cm}}
\toprule
Benchmark \& Task & Instruction Template \\ \midrule
\textbf{\lmentry{}} \\
$\quad$ all words from category & Q: Are all the words \{$words$\} types of \{$category$\}? Answer either ``yes'' or ``no''.
A:\\
 $\quad$ any words from category & Q: Does the list [\{$words$\}] contain any \{$category$\}? Answer either ``yes'' or ``no''.
A: \\
$\quad$ ends with word & Write a sentence that ends with the word ``\{$word$\}'': \\
$\quad$ first alphabetically & Q: In an alphabetical order, which word comes first, ``\{$word1$\}'' or ``\{$word2$\}''?
A: \\
$\quad$ homophones & Q: Which word sounds like the word ``\{$query$\}'', ``\{$word1$\}'' or ``\{$word2$\}''?
A: \\
$\quad$ less letters & Q: Which word is shorter, ``\{$word1$\}'' or ``\{$word2$\}''?
A: \\
$\quad$ more letters & Q: Which word has more letters, ``\{$word1$\}'' or ``\{$word2$\}''?
A: \\
$\quad$ rhyming word & Q: Which is a rhyme of the word ``\{$query$\}'', ``\{$word1$\}'' or ``\{$word2$\}''?
 A: \\
$\quad$ word before & Q: Which word comes right before ``\{$word$\}'' in the sentence ``\{$sentence$\}''?
A: \\
$\quad$ word not containing & Write a word that doesn't contain the letter ``\{$letter$\}'':
  \\\midrule

\textbf{\bigbenchlite{}}\\
$\quad$ bbq lite    &    \{$input$\}
option: \{$option1$\}
option: \{$option2$\}
option: \{$option3$\}
Answer: 
         \\
$\quad$    code line description    &  Python code:
\{$input$\}
choice: \{$option1$\}
choice: \{$option2$\}
choice: \{$option3$\}
choice: \{$option4$\}

English language description:           \\
$\quad$   conceptual combinations     &    \{$input$\}
option: \{$option1$\}
option: \{$option2$\}
option: \{$option3$\}
option: \{$option4$\}
Answer:          \\
$\quad$    hindu knowledge    &     Q: \{$input$\}
choice: \{$option1$\}
choice: \{$option2$\}
choice: \{$option3$\}
choice: \{$option4$\}
A:         \\
$\quad$   known unknown    &    \{$input$\}
choice: \{$option1$\}
choice: \{$option2$\}
          \\
$\quad$    language identification    &   Given a sentence, select the correct language among the choices
Sentence: \{$input$\}
choice: \{$option1$\}
choice: \{$option2$\}
choice: \{$option3$\}
choice: \{$option4$\}
...
Language:          \\
$\quad$     logic grid puzzle   &    \{$input$\}
                                  Answer:\\
$\quad$    logical deduction   &  The following paragraphs each describe a set of three objects arranged in a fixed order. The statements are logically consistent within each paragraph.

\{$input$\} 
           \\
$\quad$    novel concepts    &   Let's do some find-the-common-concept problems. In these problems, your goal is to identify the underlying concept or theme that relates the things listed. Make sure to answer carefully.
\{$input$\}
Answer:
          \\
$\quad$    play dialog    & The following transcripts of dialogues have been taken from Shakespeare plays, but the transcripts do not say who said what.  Your task is to identify whether the sentences in question were spoken by the same or different people.
Dialogue:
\{$input$\}
Answer:
           \\
$\quad$    strange stories     &   Context: \{$input$\}
choice: \{$option1$\}
choice: \{$option2$\}
choice: \{$option3$\}
choice: \{$option4$\}
A:
          \\
$\quad$    strategic qa    &   Q: \{$input$\}
A:
          \\
$\quad$    vitaminc fact verification    &  Based only on the information contained in a brief quote from Wikipedia, answer whether the related claim is True, False or Neither. Use Neither when the Wikipedia quote does not provide the necessary information to resolve the question.

Passage:
\{$input$\}

True, False, or Neither?
           \\
$\quad$     winowhy   &   Please answer the following questions about which words certain pronouns refer to.
\{$input$\}
The above reasoning is          \\ \midrule



 \textbf{\bigbenchhard{}} \\
$\quad$  causal judgement    & How would a typical person answer each of the following questions about causation? \\
% \{$question$\}
% Options:
% - Yes
% - No
% A:             \\
$\quad$ disambiguation qa    & In the following sentences, explain the antecedent of the pronoun (which thing the pronoun refers to), or state that it is ambiguous. \\
% Sentence: \{$sentence$\}
% Options:
% \{$options$\}
% A:            \\
$\quad$ formal fallacies   &  Is the argument, given the explicitly stated premises, deductively valid or invalid? \\
% Options:
% - valid
% - invalid
% A:           \\
$\quad$  geometric shapes    & This SVG path element \{$svg\_path\_element$\} draws a  Options: \{$options$\} \\
% A:            \\
$\quad$ hyperbaton   & Which sentence has the correct adjective order: \\
% Options:
% \{$options$\}
% A:            \\
$\quad$ logical deduction five objects    &  QThe following paragraphs each describe a set of five objects arranged in a fixed order. The statements are logically consistent within each paragraph. \\
% \{$paragraph$\}
% Options:
% \{$options$\}
% A:           \\
$\quad$ logical deduction seven objects    &  The following paragraphs each describe a set of seven objects arranged in a fixed order. The statements are logically consistent within each paragraph \\
% \{$paragraph$\}
% Options:
% \{$options$\}
% A:           \\
$\quad$  logical deduction three objects   &  The following paragraphs each describe a set of three objects arranged in a fixed order. The statements are logically consistent within each paragraph. \\
% \{$paragraph$\}
% Options:
% \{$options$\}
% A:           \\
$\quad$ movie recommendation    &  Find a movie similar to \{$movie\_list$\} \\
% Options:
% \{$options$\}
% A:           \\
$\quad$  navigate    & If you follow these instructions, do you return to the starting point? \\
% \{$instructions$\}
% Options:
% - Yes
% - No
% A:            \\
$\quad$  penguins in a table   & Here is a table where the first line is a header and each subsequent line is a penguin:  name, age, height (cm), weight (kg)  \{$question$\} \\
% \{$table\_description$\}
% \{$question$\}
% Options:
% \{$options$\}
% A:            \\
$\quad$  ruin names    & Q: Which of the following is a humorous edit of this artist or movie name: '\{$artist\_or\_movie\_name$\}'? \\
% Options:
% \{$options$\}
% A:
%             \\
$\quad$   salient translation error detection    &  The following translations from German to English contain a particular error. That error will be one of the following types: $\ldots$ Please identify that error. \\
% Source: \{$source$\}
% Translation: \{$translation$\}
% The translation contains an error pertaining to
% Options:
% \{$options$\}
% A:
%            \\
$\quad$  snarks    & Which statement is sarcastic? \\
% Options:
% \{$options$\}
% A:
%             \\
$\quad$  sports understanding    & Q: Is the following sentence plausible? \\
% ``\{$sentence$\}''
% A:
\\ \bottomrule

\end{tabular}%
%}
\caption{The 39 tasks used in this paper, along with the benchmarks from which they were taken and an example task instruction.}
\label{tab:tasks}
\end{adjustwidth}
\end{table*}

==> tables/tau_table.tex <==


\begin{table*}[bt!]
\small
\centering
%\resizebox{textwidth}{!}{
\begin{tabular}{lp{5cm}p{5cm}c}
\toprule
Task & Instruction Template \#1 & Instruction Template \#2 & $\tau$ \\ \midrule
 all words from category & 
 Can you confirm if the list [\{$words$\}] consists solely of \{$category$\}? Please respond with either "yes" or "no".
& 
Determine whether all the words in a given list belong to a specific category. The category is represented by the keyword \{$category$\}, and the list of words is represented by the keyword \{$words$\}. Answer the question with either 'yes' or 'no'.
Category: \{$category$\}
Words: \{$words$\}
Output:
& 0.029 \\
  any words from category & Is \{$category$\} represented by any of these words \{$words$\}? Respond with either 'yes' or 'no'.
  & Given a list of words, determine if any of them belong to a specific category. Respond with either "yes" or "no".
Words: \{$words$\}
Category: \{$category$\}
Output: & -0.200 \\
 ends with word & 
Provide a sentence that finishes with the term \{$word$\}. & 
Generate a sentence that ends with a specific word. Try to create a coherent sentence that effectively uses the provided word.
Word: \{$word$\}
Sentence: & -0.018 \\
 first alphabetically& 
 Which word comes first alphabetically, ``\{$word1$\}'' or ``\{$word2$\}''?
 & Please determine which of the two provided words is the first one alphabetically. The two words to be compared are denoted by placeholders \{$word1$\} and \{$word2$\}.
Word 1: \{$word1$\}
Word 2: \{$word2$\}
Output: The first word alphabetically is
& -0.095 \\
 homophones & 
 Can you tell me which word, \{$word1$\} or \{$word2$\}, sounds like \{$query$\}? & 
 Given two words, determine which one is a homophone or sounds more like a query word.
Query word: \{$query$\}
Word 1: \{$word1$\}
Word 2: \{$word2$\}
The word that sounds more like {query} is:
& 0.087 \\
 less letters & 
 Which of \{$word1$\} and \{$word2$\} has fewer letters? 
 & Compare two words and determine which one has fewer letters. The words are represented by the keywords \{$word1$\} and \{$word2$\}. Provide the keyword of the word with fewer letters.
word1: \{$word1$\}
word2: \{$word2$\}
Output keyword:
& -0.128 \\
 more letters & 
 Please compare the length of ``\{$word1$\}'' and ``\{$word2$\}'' and provide the longer word.
 & Write a program that compares the length of two words and determines which one has more letters. Your program should take two words as input and output the word with more letters. 
Word 1: \{$word1$\}
Word 2: \{$word2$\}
Output:
& -0.085 \\
 rhyming word & 
 What is a word that rhymes with `\{$query$\}', `\{$word1$\}' or `\{$word2$\}'? & 
Given a query word and two candidate words, determine which candidate word rhymes with the query word. Your response should be the candidate word that rhymes with the query word. 
Query word: \{$query$\}
Candidate word 1: \{$word1$\}
Candidate word 2: \{$word2$\}
Output word:& 0.090 \\
 word before & 
 Locate the word that comes immediately before `\{$word$\}' in the given sentence `\{$sentence$\}'
& Given a sentence and a target word, identify the word that immediately precedes the target word in the sentence.
Sentence: \{$sentence$\}
Target word: \{$word$\}
The word that comes right before \{$word$\} in the sentence is:
& -0.099 \\
 word not containing & 
 Create a term that does not have the inclusion of the letter ``\{$letter$\}''.
 & Write a word that does not contain the letter ``\{$letter$\}''.
Letter: \{$letter$\}
Output word: & -0.010 \\

\bottomrule

\end{tabular}%
%}
\caption{Kendall $\tau$ values of the disagreement between ranks on models from example paraphrases for each task in \lmentry{}.}
\label{tab:tau_lmentry}
\end{table*}



\begin{table*}[bt!]
\begin{adjustwidth}{-1cm}{-1cm}
\small
\centering
%\resizebox{textwidth}{!}{

\begin{tabular}{@{}p{1.5cm}p{7.5cm}p{7.5cm}c@{}}
\toprule
Task & Instruction Template \#1 & Instruction Template \#2 & $\tau$ \\ \midrule
  causal judgement    & You are required to give your opinion on the following question about causation: \{$question$\}. You must select either ``yes'' or ``no''. & Given a scenario, determine whether a typical person would attribute causality to a certain factor or not. Answer with ``yes'' or ``no''.
Scenario: \{$question$\}
Answer: & 0.183 \\
 disambiguation qa   & Q: For the given sentence, identify the antecedent of the ambiguous pronoun or state that it is ambiguous.
Sentence: \{$sentence$\}
Choose the option that correctly identifies the antecedent of the pronoun:
\{$options$\}
A: & Please clarify the meaning of the following sentence by selecting the option that correctly identifies the antecedent of the pronoun or state if it is ambiguous.
Sentence: \{$sentence$\}
Options:
\{$options$\}
Output: & 0.164 \\
 formal fallacies   & Q: ``Classify the argument as either a formal fallacy or deducively valid. The explicitly stated premises are \{$input$\}.''
Options:
- deductively valid
- formal fallacy & Given a set of explicitly stated premises, determine whether the argument is deductively valid or a formal fallacy. Respond with ``valid'' or ``invalid''.
Premises and conclusion: \{$input$\}
Output: & -0.264 \\
  geometric shapes  & Q: Identify the name of the geometric shape represented by the following SVG path element: \{$svg\_path\_element$\}.
Options:
\{$options$\}
A: & From the given options \{$options$\}, select the name of the geometric shape that is represented by \{$svg\_path\_element$\}. & -0.267 \\
 hyperbaton   & Order the adjectives correctly before a noun in English sentences, following the pattern of ``[1. opinion] [2. size] [3. age] [4. shape] [5. color] [6. origin] [7. material] [8. purpose] noun''. You will be presented with a multi-choice format question asking which sentence has the correct adjective order, with options provided.
Which of the following sentences has the correct adjective order?
\{$options$\} & Identify the sentence that has the correct order of adjectives in English. Choose the sentence that has the correct order of adjectives. 
Options:
\{$options$\}
Output: & 0.019 \\
 logical deduction five objects    & In this logical deduction task named logical deduction five objects, you will be given a set of paragraphs describing a set of five objects arranged in a fixed order. The statements are logically consistent within each paragraph. Your task is to choose the correct option from the given options. The options are \{$options$\}. The paragraph is \{$paragraph$\}. & Deduce the order of a sequence of five objects based on given logical statements. You will be given a set of logical statements and multiple choices for the order of the objects. Choose the correct order based on the given statements.
Statements: \{$paragraph$\}
Options:
\{$options$\}
Output: & 0.264 \\
 logical deduction seven objects    & Your task is to solve a logical deduction task which requires you to deduce the order of a sequence of objects. The task consists of a set of paragraphs, each describing a set of seven objects arranged in a fixed order. The statements are logically consistent within each paragraph. You will also be provided with multiple options to choose from. The options are represented by \{$options$\}. You should choose the correct option based on the information provided in the paragraph, which is represented by \{$paragraph$\}. & Deduce the order of a sequence of seven objects based on given statements. Use the provided options to answer each question.
Statements: \{$paragraph$\}
Options:
\{$options$\}
Output: & 0.133 \\
  logical deduction three objects   & Deduce the order of a sequence of three objects based on the logically consistent statements provided in the following \{$paragraph$\}. Choose the correct order from the given \{$options$\}. & Deduce the order of a sequence of three objects based on given statements and choose the correct option among multiple choices.
Statements: \{$paragraph$\}
Options:
\{$options$\}
Output: & 0.056 \\
 movie recommendation    & Q: Can you suggest a movie similar to \{$movie\_list$\}?
Please choose from the following options:
\{$options$\}
A: & Based on a list of movies, recommend a similar movie from a set of options. Choose the option that best matches the given list.
List of movies: \{$movie\_list$\}
Options:
\{$options$\}
Output: & -0.018 \\
  navigate  & Q: Would someone following \{$instructions$\} end up back at the starting point?
Options:
- Yes
- No
A: & Classify whether a series of navigation instructions will lead to the starting point or not. Provide either ``yes'' or ``no'' as the output. 
Instructions: \{$instructions$\}
Output: & 0.294 \\
  penguins in a table   & Please answer the following question about the table of penguins: \{$question$\} The table has a header and each subsequent line represents a penguin with attributes: name, age, height (cm), weight (kg). \{$table\_description$\} You can choose from the following options: \{$options$\} & Given a table of penguins and their attributes, answer multiple choice questions about the penguins. The prompt will include a description of the table and several options to choose from.
Table: \{$table\_description$\}
Question prompt: \{$question$\}
Options: 
\{$options$\}
Output: & 0.241 \\
  ruin names  & Which of the following options is a funny way to ``ruin'' the name of \{$artist\_or\_movie\_name$\}?
Choose from the following:
\{$options$\} & Choose the option that best 'ruins' the \{$artist\_or\_movie\_name$\}:
Options:
\{$options$\}
Answer: & 0.075 \\
  salient translation error detection & Q: Identify the type of error in the given English translation of a German source sentence. The error will belong to one of the following categories: Named Entities, Numerical Values, Modifiers or Adjectives, Negation or Antonyms, Facts, or Dropped Content. The source sentence is \{$source$\}, and its translation is \{$translation$\}. From the options below, select the category that best describes the error.
Options:
\{$options$\} & Given an English translation of a German source sentence, identify the type of error present in the translation. The error can be one of the following types: Named Entities, Numerical Values, Modifiers or Adjectives, Negation or Antonyms, Facts, or Dropped Content. You must select the correct answer from the given options in a multi-choice format.
German source sentence: \{$source$\}
English translation: \{$translation$\}
Options:
\{$options$\} & 0.389 \\
  snarks & Determine which of two sentences is sarcastic. The format is multi-choice and the prompt asks ``which statement is sarcastic?'' with two options provided. The correct option contains a taste of irony and satire. 
Options:
\{$options$\}
Output: & Given a question asking which statement is sarcastic and a list of options to choose from, determine which of the options is the sarcastic one.
Question: ``which statement is sarcastic?''
Options: 
\{$options$\}
Output: & 0.22 \\
  sports understanding  & Please classify the sentence ``\{$sentence$\}'' as either plausible or not plausible in the context of sports. & Is the following sentence plausible? \{$sentence$\}
Answer with either ``yes'' or ``no''.
Output: & -0.245 \\ 
\bottomrule

\end{tabular}%

%}
\caption{Kendall $\tau$ values of the disagreement between ranks on models from example paraphrases for each task in \bbh{}.}
\label{tab:tau_bbh}
\end{adjustwidth}
\end{table*}


\begin{table*}[bt!]
\begin{adjustwidth}{-1cm}{-1cm}
\small
\centering
%\resizebox{textwidth}{!}{
\begin{tabular}{p{1.5cm}p{7cm}p{7cm}c}
\toprule
Task & Instruction Template \#1 & Instruction Template \#2 & $\tau$ \\ \midrule
 bbq lite    & You are examined with your ability on social fairness by answering questions that contain bias content including: age, disability, gender, nationality, physical appearance, race ethnicity, religion, social status, and sexual orientation. \{$question$\}
Choose the most appropriate answer from: 
A) \{$choiceA$\}
B) \{$choiceB$\}
C) \{$choiceC$\}. & We are running a test for social biases. We will give you a question and a series of multiple-answers (A, B, C). Please choose from among the answers.

Question: \{$question$\}
A: \{$choiceA$\}
B: \{$choiceB$\}
C: \{$choiceC$\}

Answer: & 0.222 \\
    code line description    & If you are an experienced code reviewer, please give an English language description of Python code\{$question$\}. Which is the most suitable? A.  \{$choiceA$\} B.  \{$choiceB$\} C.  \{$choiceC$\} D.  \{$choiceD$\}

Answer: & You are given a simple line of Python code \{$question$\}. Try to find out its English equivalency from the following short sentences: A) \{$choiceA$\}, B) \{$choiceB$\} C) \{$choiceC$\}, D) \{$choiceD$\}. The equivalent sentence is: & 0.333 \\
   conceptual combinations     & You are a linguistic expert that knows most of the concepts and combinations of words. Now, answer the following question: \{$context$\} Question: \{$question$\} (A) \{$choiceA$\} (B) \{$choiceB$\} (C) \{$choiceC$\} (D) \{$choiceD$\}
Your answer is: & Question: \{$question$\}
The options are: 
A. \{$choiceA$\}
B. \{$choiceB$\}
C. \{$choiceC$\}
D. \{$choiceD$\}
Here is a context to help you answer the question: \{$context$\}. Choose the best answer from ``A'', ``B'', ``C'', ``D''. & 0.182 \\
    hindu knowledge   & In this task, you have to select the option that best answers the question given your knowledge about Hindu mythology.
Question: \{$question$\}
A.  \{$choiceA$\} B.  \{$choiceB$\} C.  \{$choiceC$\} D.  \{$choiceD$\}
Answer: among A, B, C, and D, the best choice is & \{$question$\}

A: \{$choiceA$\} B: \{$choiceB$\} C: \{$choiceC$\} D: \{$choiceD$\}
With your expertise inhindu mythology, provide the correct answer: & 0.444 \\
   known unknown   & Verify if the question is unknown, choose your answer from options:
Question: \{$question$\}
Options:
A: \{$choiceA$\}
B: \{$choiceB$\}
Answer: & Question: \{$question$\}
To avoid hallucination, if the answer to this question is unknown, output ``B'', otherwise output ``A'' & -0.029 \\
    language identification   & Please read the following sentence, then choose from the options which language you think it most likely came from. Your answer should be ``A'', ``B'', ``C'', ``D'', ``E'', ``F'', ``G'', ``H'', ``I'', ``J'', or ``K''
Sentence: \{$question$\}
Options:
A: \{$choiceA$\}
B: \{$choiceB$\}
C: \{$choiceC$\}
D: \{$choiceD$\}
E: \{$choiceE$\}
F: \{$choiceF$\}
G: \{$choiceG$\}
H: \{$choiceH$\}
I: \{$choiceI$\}
J: \{$choiceJ$\}
K: \{$choiceK$\}
Answer: & Please give the language used in the following sentence. Each sentence will give five options, please output the corresponding option (i.e. A, B, C, D, E, F, G, H, I, J, or K) to represent the corresponding answer.

Sentence: \{$question$\}
Options: & 0.028 \\
     logic grid puzzle   & You are given a logic grid puzzle to test your sense of space and positions. You are given a context and some clues to pick the correct answer from the options to answer a question.Context: \{$context$\}
\{$clues$\}
Question: \{$question$\}
Options:
(A) \{$choiceA$\}
(B) \{$choiceB$\}
(C) \{$choiceC$\}
(D) \{$choiceD$\}
(E) \{$choiceE$\}
Answer: & You are a master at solving logic grid puzzles. Solve this: \{$context$\}

\{$clues$\}

\{$question$\} & 0.327 \\
    logical deduction   & Given the following text describing the correct order of five objects, select the option from (A, B, C, D or E) that is consistent with the text.

text: \{$question$\}\{$options$\}

answer: & The following text describes the arrangement order of five objects. Please read the text and choose the one from the options that matches the logic of the text description. Your answer should be ``A'', ``B'', ``C'', ``D'' or ``E''.
Text: \{$question$\}\{$options$\} Answer: & 0.667 \\
    novel concepts   & You are given three objects \{$question$\}, choose the option from below where the objects share the greatest similarity. A. \{$choiceA$\} B. \{$choiceB$\} C. \{$choiceC$\} D. \{$choiceD$\} E. \{$choiceE$\} & \{$question$\}
Pick the most correct description from:
A.\{$choiceA$\}
B. \{$choiceB$\}
C. \{$choiceC$\}
D. \{$choiceD$\}
E. \{$choiceE$\}
My answer is: & 0.400 \\
    play dialog    & Now you are a dramatist. The following transcripts of dialogues are taken from Shakespeare plays, but the transcripts do not mark who said what.  Your task is to identify whether the sentences in question were spoken by the same or different people. Here is the play:
\{$play$\}
Question: In the preceding dialogue, were the lines \{$line1$\} and \{$line2$\} spoken by the same person or different people? Please just give a short answer: same or different.

Your Answer: & In the context of the Shakespeare play, \{$play$\}, assess the given dialogue transcripts. Determine whether the sentences \{$line1$\} and \{$line2$\} were spoken by a single person or by different people.
Answer: & -0.638 \\
    strange stories    & Given a story, answer whether the question is true or false.
\{$context$\}
Q: \{$question$\}
A: & Image you are taking a psychology test. Please read the given story and answer the question. Please answer ``yes'' or ``no''.
Story: \{$context$\}
Q: \{$question$\}
A: & 0.310 \\
    strategic qa    & Reason about the answer to the question. \{$question$\} & Please answer the following question, you should think step by step, but please use ``yes'' or ``no'' to answer.Question: \{$question$\}Answer: & -0.085 \\
    vitaminc fact verification    & Input: \{$claim$\}
Verify the factually of the claim based on the following context
\{$context$\}

- ``True'' if the claim is factually correct
- ``False'' if the claim is factually incorrect
- ``Neither'' if the factuality cannot be determined. Output you answer with one of ``True'', ``False'', or ``Neither''. Answer: & Context: \{$context$\}
Now classify this claim into one of 'True', 'False', or 'Neither'.
\{$claim$\} & 0.556 \\
     winowhy   & Read the following reasoning about who a particular pronoun refers to: \{$question$\}
Is the reasoning correct? & Read the following reasoning, and answer if its correct or incorrect. \{$question$\} & -0.056 \\ 
\bottomrule

\end{tabular}%
%}
\caption{Kendall $\tau$ values of the disagreement between ranks on models from example paraphrases for each task in \bbl{}.}
\label{tab:tau_bbl}
\end{adjustwidth}
\end{table*}

==> tables/try.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccc}
                       & \textbf{t03b}                 & \textbf{t0pp}                 & \textbf{fal7b}               & \textbf{mpt7b}               & \textbf{alp7b}               & \textbf{alp13b}               & \textbf{ft5-s}                & \textbf{ft5-b}                & \textbf{ft5-l}                & \textbf{ft5-xl}               & \textbf{ft5-xxl}              & \textbf{air13b}               & \textbf{nou13b}               & \textbf{ult13b}              & \textbf{vic13b}               & \textbf{min15b}              \\
+ `.'                  & \cellcolor[HTML]{FEF6F6}-0.01 & \cellcolor[HTML]{FBB6B7}-0.07 & \cellcolor[HTML]{7CC990}0.13 & \cellcolor[HTML]{EEF8F0}0.02 & \cellcolor[HTML]{FEFAFA}0.00 & \cellcolor[HTML]{63BE7B}0.16  & \cellcolor[HTML]{FDE4E4}-0.03 & \cellcolor[HTML]{FEFCFC}0.00  & \cellcolor[HTML]{FDE7E8}-0.02 & \cellcolor[HTML]{F98081}-0.13 & \cellcolor[HTML]{F7FCF9}0.01  & \cellcolor[HTML]{FEF9F9}-0.01 & \cellcolor[HTML]{FEEDED}-0.02 & \cellcolor[HTML]{C5E7CE}0.06 & \cellcolor[HTML]{FAFDFB}0.01  & \cellcolor[HTML]{F1F9F3}0.01 \\
`.' --\textgreater `:' & \cellcolor[HTML]{FEFDFD}0.00  & \cellcolor[HTML]{CEEBD6}0.05  & \cellcolor[HTML]{F8FDF9}0.01 & \cellcolor[HTML]{F5FBF6}0.01 & \cellcolor[HTML]{C2E6CB}0.06 & \cellcolor[HTML]{F8696B}-0.19 & \cellcolor[HTML]{F7FCF8}0.01  & \cellcolor[HTML]{FEECED}-0.02 & \cellcolor[HTML]{EFF9F2}0.02  & \cellcolor[HTML]{FDFFFE}0.00  & \cellcolor[HTML]{FEF4F4}-0.01 & \cellcolor[HTML]{FEFDFD}0.00  & \cellcolor[HTML]{B9E2C4}0.07  & \cellcolor[HTML]{FEFCFC}0.00 & \cellcolor[HTML]{FEF3F3}-0.01 & \cellcolor[HTML]{FEFAFA}0.00
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}
